Monotone Cubic B-Splines with a Neural-Network Generator

We present a method for fitting monotone curves using cubic B-splines, which is equivalent to putting a monotonicity constraint on the coefficients. We explore different ways of enforcing this constraint and analyze their theoretical and empirical properties. We propose two algorithms for solving the spline fitting problem: one that uses standard optimization techniques and one that trains a Multi-Layer Perceptrons (MLP) generator to approximate the solutions under various settings and perturbations. The generator approach can speed up the fitting process when we need to solve the problem repeatedly, such as when constructing confidence bands using bootstrap. We evaluate our method against several existing methods, some of which do not use the monotonicity constraint, on some monotone curves with varying noise levels. We demonstrate that our method outperforms the other methods, especially in high-noise scenarios. We also apply our method to analyze the polarization-hole phenomenon during star formation in astrophysics. The source code is accessible at \texttt{\url{https://github.com/szcf-weiya/MonotoneSplines.jl}}.

==> res/acc_monofit/2b5310d/10x15w-prop0.2-eta01e-4/res.tex <==
\begin{tabular}{cccccccccccccccccccccc}
\toprule
\multirow{2}{*}{noise} & \multirow{2}{*}{curve}&\multicolumn{10}{c}{Relative Gap}&\multicolumn{10}{c}{Fittness Ratio}\tabularnewline
\cmidrule(lr){3-12}
\cmidrule(lr){13-22}
&&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$\tabularnewline
\midrule
\midrule
\multirow{4}{*}{sigma = 0.02}&logit5&8.40e-04&5.89e-04&3.81e-04&1.90e-04&3.76e-05&9.24e-06&7.56e-06&4.96e-07&6.88e-08&2.68e-07&2.05e+00&1.71e+00&1.40e+00&1.12e+00&9.83e-01&1.10e+00&1.07e+00&9.88e-01&9.99e-01&9.99e-01\tabularnewline
&exp&1.71e-04&7.78e-05&2.67e-05&5.52e-06&8.68e-07&9.93e-07&4.13e-07&3.86e-08&1.46e-08&5.98e-08&1.82e+00&1.36e+00&1.12e+00&1.02e+00&1.01e+00&1.03e+00&1.02e+00&1.00e+00&9.98e-01&1.00e+00\tabularnewline
&cubic&2.22e-03&7.55e-04&1.83e-04&3.90e-05&9.12e-06&1.16e-05&4.72e-06&1.73e-06&2.31e-07&7.46e-07&1.91e+00&1.28e+00&1.04e+00&1.00e+00&1.02e+00&1.04e+00&1.01e+00&9.94e-01&1.00e+00&1.00e+00\tabularnewline
&sinhalfpi&5.95e-04&3.38e-04&1.50e-04&4.23e-05&1.88e-06&6.68e-06&2.93e-06&4.67e-07&7.00e-08&2.52e-07&1.83e+00&1.44e+00&1.16e+00&1.01e+00&1.00e+00&1.07e+00&1.04e+00&9.87e-01&1.00e+00&1.00e+00\tabularnewline
\midrule
\multirow{4}{*}{sigma = 0.1}&logit5&8.28e-04&5.85e-04&3.26e-04&1.38e-04&2.81e-05&1.40e-05&1.09e-05&8.99e-07&1.67e-07&5.33e-07&1.05e+00&1.04e+00&1.02e+00&1.01e+00&1.00e+00&1.01e+00&1.01e+00&9.96e-01&1.00e+00&1.00e+00\tabularnewline
&exp&1.86e-04&7.79e-05&2.33e-05&4.01e-06&1.03e-06&8.07e-07&2.19e-07&5.89e-08&1.59e-08&5.19e-08&1.06e+00&1.03e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&9.99e-01&1.00e+00\tabularnewline
&cubic&2.16e-03&7.96e-04&1.86e-04&7.25e-05&4.85e-05&9.30e-06&3.53e-06&1.25e-06&2.20e-07&4.57e-07&1.05e+00&1.02e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&9.97e-01&1.00e+00&1.00e+00\tabularnewline
&sinhalfpi&5.32e-04&2.81e-04&1.16e-04&3.08e-05&4.69e-06&6.01e-06&1.93e-06&6.65e-07&6.77e-08&3.09e-07&1.05e+00&1.03e+00&1.01e+00&1.01e+00&1.00e+00&1.01e+00&1.01e+00&9.96e-01&1.00e+00&1.00e+00\tabularnewline
\midrule
\multirow{4}{*}{sigma = 0.2}&logit5&1.14e-03&6.86e-04&4.02e-04&1.52e-04&3.36e-05&1.74e-05&1.18e-05&1.07e-06&8.70e-08&4.08e-07&1.02e+00&1.01e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&9.99e-01&1.00e+00&1.00e+00\tabularnewline
&exp&2.73e-04&1.11e-04&3.20e-05&5.67e-06&1.49e-06&1.11e-06&2.41e-07&9.63e-08&2.86e-08&8.42e-08&1.03e+00&1.02e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00\tabularnewline
&cubic&2.65e-03&8.26e-04&1.83e-04&4.79e-05&3.34e-05&9.60e-06&5.17e-06&1.25e-06&1.79e-07&6.56e-07&1.03e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&9.99e-01&1.00e+00&1.00e+00\tabularnewline
&sinhalfpi&9.94e-04&4.59e-04&1.86e-04&4.08e-05&1.04e-05&1.18e-05&2.89e-06&5.80e-07&5.71e-08&2.82e-07&1.02e+00&1.01e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&9.99e-01&1.00e+00&1.00e+00\tabularnewline
\midrule
\multirow{4}{*}{sigma = 0.5}&logit5&2.81e-03&9.41e-04&2.38e-04&1.22e-04&1.03e-04&1.66e-05&4.25e-06&8.85e-07&1.95e-07&6.39e-07&1.01e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00\tabularnewline
&exp&6.82e-04&1.94e-04&6.46e-05&1.62e-05&5.16e-06&1.32e-06&3.23e-07&7.81e-08&1.52e-08&1.18e-07&1.02e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00\tabularnewline
&cubic&3.59e-03&9.27e-04&3.08e-04&1.36e-04&6.31e-05&2.74e-05&5.80e-06&1.74e-06&1.26e-07&4.52e-07&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00\tabularnewline
&sinhalfpi&1.87e-03&7.63e-04&2.53e-04&6.67e-05&1.79e-05&1.18e-05&1.75e-06&6.63e-07&8.39e-08&2.20e-07&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00\tabularnewline
\bottomrule
\end{tabular}


==> res/acc_monofit/2b5310d/10x15w-prop0.2-eta01e-4/res_simplify.tex <==
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{noise} & \multirow{2}{*}{curve}&\multicolumn{3}{c}{Relative Gap}&\multicolumn{3}{c}{Fitness Ratio}\tabularnewline
\cmidrule(lr){3-5}
\cmidrule(lr){6-8}
&&$\lambda_l$&$\lambda_u$&Avg.&$\lambda_l$&$\lambda_u$&Avg.\tabularnewline
\midrule
\multirow{4}{*}{$\sigma = 0.1$}&$S(5x)$& 8.28e-04 (4.3e-04)& 5.33e-07 (3.9e-07)& 1.93e-04 (3.4e-04)& 1.05e+00 (2.3e-02)& 1.00e+00 (3.6e-03)& 1.01e+00 (2.1e-02)\tabularnewline
&$e^x$& 1.86e-04 (7.9e-05)& 5.19e-08 (4.8e-08)& 2.93e-05 (6.3e-05)& 1.06e+00 (2.4e-02)& 1.00e+00 (2.4e-03)& 1.01e+00 (2.0e-02)\tabularnewline
&$x^3$& 2.16e-03 (9.1e-04)& 4.57e-07 (4.0e-07)& 3.28e-04 (7.3e-04)& 1.05e+00 (2.2e-02)& 1.00e+00 (1.6e-03)& 1.01e+00 (1.6e-02)\tabularnewline
&$\sin(\pi x/2)$& 5.32e-04 (2.8e-04)& 3.09e-07 (1.7e-07)& 9.74e-05 (2.0e-04)& 1.05e+00 (2.4e-02)& 1.00e+00 (1.6e-03)& 1.01e+00 (1.8e-02)\tabularnewline
\midrule
\multirow{4}{*}{$\sigma = 0.2$}&$S(5x)$& 1.14e-03 (3.5e-04)& 4.08e-07 (1.6e-07)& 2.45e-04 (3.9e-04)& 1.02e+00 (8.6e-03)& 1.00e+00 (8.9e-04)& 1.01e+00 (8.5e-03)\tabularnewline
&$e^x$& 2.73e-04 (1.2e-04)& 8.42e-08 (6.4e-08)& 4.25e-05 (9.4e-05)& 1.03e+00 (1.3e-02)& 1.00e+00 (1.2e-03)& 1.01e+00 (9.6e-03)\tabularnewline
&$x^3$& 2.65e-03 (1.7e-03)& 6.56e-07 (8.6e-07)& 3.75e-04 (9.8e-04)& 1.03e+00 (1.6e-02)& 1.00e+00 (1.1e-03)& 1.00e+00 (9.6e-03)\tabularnewline
&$\sin(\pi x/2)$& 9.94e-04 (5.7e-04)& 2.82e-07 (2.0e-07)& 1.71e-04 (3.7e-04)& 1.02e+00 (9.2e-03)& 1.00e+00 (9.5e-04)& 1.01e+00 (8.1e-03)\tabularnewline
\midrule
\multirow{4}{*}{$\sigma = 0.5$}&$S(5x)$& 2.81e-03 (1.6e-03)& 6.39e-07 (9.8e-07)& 4.23e-04 (9.9e-04)& 1.01e+00 (9.2e-03)& 1.00e+00 (2.5e-04)& 1.00e+00 (5.1e-03)\tabularnewline
&$e^x$& 6.82e-04 (4.9e-04)& 1.18e-07 (1.1e-07)& 9.65e-05 (2.6e-04)& 1.02e+00 (1.1e-02)& 1.00e+00 (1.6e-04)& 1.00e+00 (6.7e-03)\tabularnewline
&$x^3$& 3.59e-03 (2.7e-03)& 4.52e-07 (3.8e-07)& 5.06e-04 (1.4e-03)& 1.01e+00 (4.1e-03)& 1.00e+00 (2.0e-04)& 1.00e+00 (3.0e-03)\tabularnewline
&$\sin(\pi x/2)$& 1.87e-03 (9.9e-04)& 2.20e-07 (1.7e-07)& 2.99e-04 (6.6e-04)& 1.01e+00 (1.2e-02)& 1.00e+00 (2.2e-04)& 1.00e+00 (5.1e-03)\tabularnewline
\bottomrule
\end{tabular}


==> res/acc_monofit/2b5310d/5x15w-prop0.2-eta01e-4/res.tex <==
\begin{tabular}{cccccccccccccccccccccc}
\toprule
\multirow{2}{*}{noise} & \multirow{2}{*}{curve}&\multicolumn{10}{c}{Relative Gap}&\multicolumn{10}{c}{Fittness Ratio}\tabularnewline
\cmidrule(lr){3-12}
\cmidrule(lr){13-22}
&&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$\tabularnewline
\midrule
\midrule
\multirow{3}{*}{sigma = 0.1}&logit5&6.32e-04&3.90e-04&2.18e-04&6.99e-05&1.04e-05&1.23e-05&4.72e-06&8.91e-07&1.07e-07&3.05e-07&1.04e+00&1.02e+00&1.01e+00&1.00e+00&1.00e+00&1.01e+00&1.01e+00&9.95e-01&1.00e+00&1.00e+00\tabularnewline
&exp&2.84e-04&1.25e-04&3.65e-05&6.63e-06&1.59e-06&1.15e-06&3.80e-07&4.37e-08&1.37e-08&8.93e-08&1.08e+00&1.04e+00&1.02e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00\tabularnewline
&cubic&2.08e-03&7.50e-04&2.01e-04&3.85e-05&1.95e-05&8.39e-06&3.76e-06&1.49e-06&2.02e-07&9.01e-07&1.04e+00&1.02e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&9.98e-01&1.00e+00&1.00e+00\tabularnewline
\midrule
\multirow{3}{*}{sigma = 0.2}&logit5&8.63e-04&5.43e-04&3.84e-04&2.42e-04&5.43e-05&1.85e-05&6.86e-06&1.06e-06&9.84e-08&4.38e-07&1.02e+00&1.01e+00&1.01e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&9.99e-01&1.00e+00&1.00e+00\tabularnewline
&exp&3.71e-04&1.47e-04&3.09e-05&4.86e-06&3.40e-06&1.12e-06&2.03e-07&8.72e-08&2.61e-08&1.33e-07&1.03e+00&1.01e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00\tabularnewline
&cubic&1.33e-03&5.52e-04&1.90e-04&3.24e-05&2.91e-05&5.16e-06&3.50e-06&5.37e-07&1.66e-07&5.04e-07&1.02e+00&1.01e+00&1.01e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&1.00e+00&9.99e-01\tabularnewline
\bottomrule
\end{tabular}


==> res/acc_monofit/2b5310d/5x15w-prop0.2/res.tex <==
\begin{tabular}{cccccccccccccccccccccc}
\toprule
\multirow{2}{*}{noise} & \multirow{2}{*}{curve}&\multicolumn{10}{c}{Relative Gap}&\multicolumn{10}{c}{Fittness Ratio}\tabularnewline
\cmidrule(lr){3-12}
\cmidrule(lr){13-22}
&&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$\tabularnewline
\midrule
\midrule
\multirow{3}{*}{sigma = 0.1}&logit5&7.64e-03&3.76e-03&1.83e-03&8.86e-04&3.20e-04&1.69e-04&7.31e-05&4.78e-06&1.37e-06&7.55e-06&1.31e+00&1.17e+00&1.09e+00&1.04e+00&1.02e+00&1.03e+00&1.03e+00&1.00e+00&9.95e-01&9.97e-01\tabularnewline
&exp&2.90e-03&1.71e-03&9.28e-04&4.34e-04&1.50e-04&3.00e-05&1.47e-05&1.14e-05&1.06e-06&6.36e-06&1.63e+00&1.38e+00&1.21e+00&1.10e+00&1.04e+00&1.02e+00&1.02e+00&1.03e+00&9.88e-01&1.03e+00\tabularnewline
&cubic&2.00e-02&1.28e-02&6.57e-03&2.48e-03&4.79e-04&1.46e-04&2.03e-04&4.02e-06&3.48e-06&8.54e-06&1.34e+00&1.23e+00&1.12e+00&1.04e+00&1.01e+00&1.03e+00&1.04e+00&9.97e-01&9.95e-01&9.94e-01\tabularnewline
\midrule
\multirow{3}{*}{sigma = 0.2}&logit5&4.71e-03&2.71e-03&1.78e-03&9.78e-04&2.39e-04&4.19e-05&5.67e-05&1.43e-05&2.85e-06&9.36e-06&1.08e+00&1.05e+00&1.04e+00&1.03e+00&1.01e+00&1.01e+00&1.01e+00&1.00e+00&9.98e-01&1.00e+00\tabularnewline
&exp&2.67e-03&1.81e-03&9.88e-04&4.17e-04&1.20e-04&1.60e-05&1.15e-05&9.90e-06&1.06e-06&5.35e-06&1.16e+00&1.12e+00&1.08e+00&1.04e+00&1.02e+00&1.01e+00&1.00e+00&1.01e+00&9.96e-01&1.01e+00\tabularnewline
&cubic&2.24e-02&1.53e-02&1.06e-02&3.70e-03&5.65e-04&1.86e-04&2.91e-04&4.69e-06&5.48e-06&1.58e-05&1.13e+00&1.10e+00&1.07e+00&1.03e+00&1.01e+00&1.01e+00&1.02e+00&1.00e+00&9.97e-01&9.97e-01\tabularnewline
\bottomrule
\end{tabular}


==> res/acc_monofit/2b5310d/5x15w-prop0.5-eta01e-4/res.tex <==
\begin{tabular}{cccccccccccccccccccccc}
\toprule
\multirow{2}{*}{noise} & \multirow{2}{*}{curve}&\multicolumn{10}{c}{Relative Gap}&\multicolumn{10}{c}{Fittness Ratio}\tabularnewline
\cmidrule(lr){3-12}
\cmidrule(lr){13-22}
&&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$\tabularnewline
\midrule
\midrule
\multirow{3}{*}{sigma = 0.1}&logit5&4.26e-03&2.82e-03&1.91e-03&9.85e-04&3.19e-04&2.24e-04&1.37e-04&3.05e-05&1.43e-04&6.86e-04&1.22e+00&1.15e+00&1.10e+00&1.05e+00&1.02e+00&1.03e+00&1.04e+00&1.01e+00&9.92e-01&1.02e+00\tabularnewline
&exp&2.77e-03&1.73e-03&9.48e-04&4.28e-04&1.50e-04&6.51e-05&8.03e-05&6.61e-05&2.59e-05&1.08e-04&1.75e+00&1.46e+00&1.25e+00&1.12e+00&1.05e+00&1.03e+00&1.05e+00&1.06e+00&1.02e+00&1.05e+00\tabularnewline
&cubic&3.05e-02&1.73e-02&7.95e-03&2.67e-03&4.40e-04&4.00e-04&3.67e-04&5.96e-05&1.66e-04&7.66e-04&1.46e+00&1.25e+00&1.11e+00&1.03e+00&1.01e+00&1.04e+00&1.05e+00&1.00e+00&9.98e-01&1.00e+00\tabularnewline
\midrule
\multirow{3}{*}{sigma = 0.2}&logit5&3.39e-03&2.31e-03&1.54e-03&7.24e-04&1.40e-04&3.56e-05&8.24e-05&4.57e-06&6.38e-06&3.46e-05&1.07e+00&1.05e+00&1.03e+00&1.02e+00&1.01e+00&1.01e+00&1.01e+00&1.00e+00&9.98e-01&9.99e-01\tabularnewline
&exp&3.58e-03&2.35e-03&1.47e-03&9.95e-04&7.97e-04&7.57e-04&7.24e-04&5.59e-04&5.09e-04&2.21e-03&1.31e+00&1.21e+00&1.14e+00&1.09e+00&1.07e+00&1.07e+00&1.07e+00&1.07e+00&1.06e+00&1.11e+00\tabularnewline
&cubic&3.43e-02&2.18e-02&1.25e-02&5.89e-03&1.25e-03&2.35e-04&2.98e-04&8.38e-06&3.64e-05&2.01e-04&1.20e+00&1.13e+00&1.07e+00&1.04e+00&1.02e+00&1.01e+00&1.02e+00&1.00e+00&9.98e-01&9.98e-01\tabularnewline
\bottomrule
\end{tabular}


==> res/acc_monofit/2b5310d/5x30w-prop0.5-eta01e-4/res.tex <==
\begin{tabular}{cccccccccccccccccccccc}
\toprule
\multirow{2}{*}{noise} & \multirow{2}{*}{curve}&\multicolumn{10}{c}{Relative Gap}&\multicolumn{10}{c}{Fittness Ratio}\tabularnewline
\cmidrule(lr){3-12}
\cmidrule(lr){13-22}
&&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$&$\lambda_{1}$&$\lambda_{2}$&$\lambda_{3}$&$\lambda_{4}$&$\lambda_{5}$&$\lambda_{6}$&$\lambda_{7}$&$\lambda_{8}$&$\lambda_{9}$&$\lambda_{10}$\tabularnewline
\midrule
\midrule
\multirow{3}{*}{sigma = 0.1}&logit5&2.41e-03&1.98e-03&1.42e-03&6.23e-04&9.43e-05&3.15e-05&4.12e-05&2.58e-06&6.48e-06&4.19e-05&1.15e+00&1.12e+00&1.08e+00&1.03e+00&1.00e+00&1.01e+00&1.02e+00&1.00e+00&9.95e-01&9.96e-01\tabularnewline
&exp&3.28e-03&2.05e-03&1.15e-03&5.34e-04&1.75e-04&3.02e-05&1.91e-05&1.96e-05&7.16e-06&6.62e-05&1.74e+00&1.45e+00&1.25e+00&1.12e+00&1.05e+00&1.02e+00&1.03e+00&1.03e+00&1.00e+00&1.05e+00\tabularnewline
&cubic&1.63e-02&9.82e-03&5.24e-03&2.16e-03&3.38e-04&1.63e-04&1.68e-04&1.15e-05&4.26e-05&2.51e-04&1.36e+00&1.20e+00&1.09e+00&1.03e+00&1.00e+00&1.03e+00&1.04e+00&9.99e-01&9.98e-01&9.98e-01\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/2022-07-04T11_07_25+08_00_logit_and_growth.tex <==
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{level0} & \multirow{2}{*}{level1}&\multicolumn{2}{c}{Logistic Curve}&\multicolumn{2}{c}{Growth Curve}\tabularnewline
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&&MSFE&MSPE&MSFE&MSPE\tabularnewline
\midrule
\multirow{13}{*}{0.1}&MQB& 9.86e-03 (2.9e-04)& 2.48e-03 (1.3e-04)& 7.68e-03 (3.9e-04)& 1.15e-02 (5.4e-04)\tabularnewline
&QB& 8.78e-03 (2.4e-04)& 1.61e-03 (8.3e-05)& 3.96e-02 (5.6e-03)& 3.68e-02 (4.5e-03)\tabularnewline
&LOESS& 8.48e-03 (2.3e-04)& 1.45e-03 (8.0e-05)& 1.35e+00 (2.0e-02)& 8.84e-01 (1.4e-02)\tabularnewline
&Isotonic& 4.62e-03 (1.7e-04)& 3.01e-03 (1.2e-04)& 3.30e-04 (4.0e-05)& 2.25e-02 (1.3e-03)\tabularnewline
&SI& 8.57e-03 (2.3e-04)& \textbf{1.33e-03} (8.0e-05)& 1.35e+00 (2.0e-02)& 9.01e-01 (1.5e-02)\tabularnewline
&IS& 8.78e-03 (2.3e-04)& 1.49e-03 (8.7e-05)& 1.35e+00 (2.0e-02)& 8.84e-01 (1.4e-02)\tabularnewline
&MONMLP (2x2)& 7.03e-03 (2.2e-04)& 2.78e-03 (1.4e-04)& 9.20e-03 (2.8e-04)& \textbf{3.51e-03} (1.6e-04)\tabularnewline
&MONMLP (4x2)& 6.31e-03 (2.1e-04)& 3.39e-03 (1.5e-04)& 7.41e-03 (2.1e-04)& 3.78e-03 (3.0e-04)\tabularnewline
&MONMLP (32x2)& 6.21e-03 (2.2e-04)& 3.57e-03 (1.7e-04)& 7.21e-03 (2.5e-04)& 5.62e-03 (1.4e-03)\tabularnewline
&MCB1& 1.11e-02 (3.0e-04)& 2.88e-03 (9.0e-05)& 5.29e-03 (2.3e-04)& 5.65e-03 (1.9e-04)\tabularnewline
&MCB2& 6.72e-03 (2.7e-04)& 2.49e-03 (1.3e-04)& 1.40e-03 (8.7e-05)& 3.60e-02 (4.0e-03)\tabularnewline
&CB1& 9.12e-03 (2.6e-04)& 1.90e-03 (8.5e-05)& 5.19e-03 (2.4e-04)& 5.95e-03 (1.9e-04)\tabularnewline
&CB2& 4.37e-03 (3.7e-04)& 3.26e-01 (1.6e-01)& 3.04e-04 (5.8e-05)& 9.55e-01 (2.3e-01)\tabularnewline
\midrule
\multirow{13}{*}{1.5}&MQB& 2.17e+00 (6.3e-02)& 2.24e-01 (2.3e-02)& 2.91e+00 (1.1e-01)& 1.01e+00 (4.1e-02)\tabularnewline
&QB& 2.02e+00 (5.7e-02)& 2.57e-01 (2.0e-02)& 3.83e+00 (1.1e-01)& 1.68e+00 (5.8e-02)\tabularnewline
&LOESS& 1.83e+00 (5.5e-02)& 3.73e-01 (2.4e-02)& 3.18e+00 (7.6e-02)& 1.13e+00 (3.5e-02)\tabularnewline
&Isotonic& 1.77e+00 (5.5e-02)& 3.24e-01 (2.4e-02)& 9.88e-01 (3.9e-02)& 6.86e-01 (2.5e-02)\tabularnewline
&SI& 1.97e+00 (5.8e-02)& 2.25e-01 (1.9e-02)& 3.19e+00 (7.6e-02)& 1.14e+00 (3.5e-02)\tabularnewline
&IS& 2.02e+00 (6.0e-02)& 2.74e-01 (2.2e-02)& 3.25e+00 (7.7e-02)& 1.14e+00 (3.6e-02)\tabularnewline
&MONMLP (2x2)& 1.87e+00 (5.8e-02)& 3.33e-01 (2.5e-02)& 1.61e+00 (4.9e-02)& 7.12e-01 (4.9e-02)\tabularnewline
&MONMLP (4x2)& 1.86e+00 (5.8e-02)& 3.30e-01 (2.4e-02)& 1.44e+00 (4.7e-02)& 7.96e-01 (4.1e-02)\tabularnewline
&MONMLP (32x2)& 1.97e+00 (6.0e-02)& 2.49e-01 (2.3e-02)& 1.44e+00 (5.1e-02)& 8.08e-01 (4.3e-02)\tabularnewline
&MCB1& 2.02e+00 (5.8e-02)& \textbf{1.99e-01} (1.8e-02)& 1.86e+00 (6.0e-02)& \textbf{4.89e-01} (2.1e-02)\tabularnewline
&MCB2& 1.90e+00 (5.8e-02)& 2.60e-01 (2.0e-02)& 1.36e+00 (5.7e-02)& 6.40e-01 (2.5e-02)\tabularnewline
&CB1& 1.85e+00 (5.6e-02)& 4.05e-01 (3.2e-02)& 1.76e+00 (5.6e-02)& 6.22e-01 (2.6e-02)\tabularnewline
&CB2& 1.14e+00 (9.1e-02)& 4.38e+01 (1.7e+01)& 8.48e-01 (8.0e-02)& 2.48e+01 (1.2e+01)\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/2022-07-04T12_19_32+08_00_cubic_and_steps.tex <==
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Noise} & \multirow{2}{*}{Method}&\multicolumn{2}{c}{Cubic Curve}&\multicolumn{2}{c}{Step Curve}\tabularnewline
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&&MSFE&MSPE&MSFE&MSPE\tabularnewline
\midrule
\multirow{13}{*}{0.1}&MQB& 9.25e-03 (8.6e-05)& 2.57e-03 (5.2e-05)& 1.33e-01 (2.1e-03)& 1.44e-01 (1.7e-03)\tabularnewline
&QB& 8.47e-03 (7.5e-05)& 1.70e-03 (3.2e-05)& 1.47e-01 (2.2e-03)& 1.57e-01 (1.8e-03)\tabularnewline
&LOESS& 8.83e-03 (7.5e-05)& 1.89e-03 (3.3e-05)& 2.29e-01 (2.4e-03)& 2.27e-01 (2.2e-03)\tabularnewline
&Isotonic& 3.81e-03 (5.1e-05)& 3.52e-03 (4.0e-05)& 4.66e-03 (6.1e-05)& \textbf{5.45e-02} (4.0e-04)\tabularnewline
&SI& 8.90e-03 (7.5e-05)& 1.85e-03 (3.4e-05)& 2.28e-01 (2.4e-03)& 2.27e-01 (2.2e-03)\tabularnewline
&IS& 9.25e-03 (7.7e-05)& 2.03e-03 (3.6e-05)& 2.30e-01 (2.4e-03)& 2.28e-01 (2.2e-03)\tabularnewline
&MONMLP (2x2)& 1.46e-02 (3.9e-04)& 7.86e-03 (3.0e-04)& 1.38e-01 (3.2e-03)& 1.59e-01 (3.0e-03)\tabularnewline
&MONMLP (4x2)& 1.30e-02 (3.8e-04)& 6.90e-03 (2.7e-04)& 1.02e-01 (2.9e-03)& 1.34e-01 (2.6e-03)\tabularnewline
&MONMLP (32x2)& 8.10e-03 (2.1e-04)& 4.54e-03 (1.6e-04)& 8.32e-02 (2.8e-03)& 1.30e-01 (2.4e-03)\tabularnewline
&MCB1& 8.61e-03 (7.7e-05)& \textbf{1.40e-03} (3.2e-05)& 2.37e-01 (3.9e-03)& 2.39e-01 (3.7e-03)\tabularnewline
&MCB2& 5.98e-03 (8.3e-05)& 2.95e-03 (4.9e-05)& 3.19e-02 (4.6e-04)& 6.79e-02 (4.8e-04)\tabularnewline
&CB1& 8.25e-03 (7.4e-05)& 1.66e-03 (3.4e-05)& 2.17e-01 (3.6e-03)& 2.19e-01 (3.3e-03)\tabularnewline
&CB2& 3.91e-03 (1.1e-04)& 2.20e-01 (3.8e-02)& 3.44e-03 (2.0e-04)& 8.96e+00 (1.0e+00)\tabularnewline
\midrule
\multirow{13}{*}{1.0}&MQB& 9.51e-01 (8.3e-03)& 1.31e-01 (3.2e-03)& 1.22e+00 (1.2e-02)& 4.88e-01 (6.1e-03)\tabularnewline
&QB& 8.92e-01 (7.9e-03)& 1.20e-01 (2.5e-03)& 1.16e+00 (1.1e-02)& 4.35e-01 (4.9e-03)\tabularnewline
&LOESS& 8.06e-01 (7.3e-03)& 1.39e-01 (2.9e-03)& 1.06e+00 (9.4e-03)& 3.68e-01 (3.8e-03)\tabularnewline
&Isotonic& 7.16e-01 (7.0e-03)& 1.38e-01 (2.8e-03)& 5.32e-01 (6.3e-03)& 3.53e-01 (3.9e-03)\tabularnewline
&SI& 8.40e-01 (7.5e-03)& 1.01e-01 (2.2e-03)& 1.06e+00 (9.4e-03)& 3.64e-01 (3.8e-03)\tabularnewline
&IS& 8.65e-01 (7.7e-03)& 1.08e-01 (2.6e-03)& 1.09e+00 (9.8e-03)& 3.69e-01 (3.8e-03)\tabularnewline
&MONMLP (2x2)& 7.89e-01 (7.5e-03)& 1.62e-01 (2.9e-03)& 8.78e-01 (1.0e-02)& 4.15e-01 (4.9e-03)\tabularnewline
&MONMLP (4x2)& 7.83e-01 (7.5e-03)& 1.63e-01 (2.9e-03)& 7.99e-01 (9.3e-03)& 4.21e-01 (5.0e-03)\tabularnewline
&MONMLP (32x2)& 9.02e-01 (8.4e-03)& 1.63e-01 (2.6e-03)& 7.84e-01 (1.1e-02)& 4.59e-01 (6.3e-03)\tabularnewline
&MCB1& 8.61e-01 (7.7e-03)& \textbf{9.76e-02} (2.2e-03)& 1.11e+00 (1.1e-02)& 3.97e-01 (4.6e-03)\tabularnewline
&MCB2& 7.88e-01 (7.6e-03)& 1.20e-01 (2.5e-03)& 7.15e-01 (8.3e-03)& \textbf{3.46e-01} (3.7e-03)\tabularnewline
&CB1& 8.13e-01 (7.7e-03)& 1.51e-01 (3.6e-03)& 1.06e+00 (1.0e-02)& 4.08e-01 (4.6e-03)\tabularnewline
&CB2& 5.13e-01 (1.1e-02)& 2.93e+01 (5.3e+00)& 3.43e-01 (1.1e-02)& 2.87e+01 (3.8e+00)\tabularnewline
\midrule
\multirow{13}{*}{1.5}&MQB& 2.18e+00 (1.9e-02)& 2.41e-01 (7.1e-03)& 2.47e+00 (2.2e-02)& 7.32e-01 (1.1e-02)\tabularnewline
&QB& 2.05e+00 (1.8e-02)& 2.27e-01 (5.5e-03)& 2.32e+00 (2.1e-02)& 6.20e-01 (8.3e-03)\tabularnewline
&LOESS& 1.87e+00 (1.7e-02)& 3.04e-01 (6.3e-03)& 2.10e+00 (1.8e-02)& 5.49e-01 (7.3e-03)\tabularnewline
&Isotonic& 1.75e+00 (1.7e-02)& 2.71e-01 (6.3e-03)& 1.29e+00 (1.4e-02)& 6.36e-01 (7.9e-03)\tabularnewline
&SI& 1.97e+00 (1.8e-02)& 1.92e-01 (5.0e-03)& 2.10e+00 (1.8e-02)& 5.36e-01 (7.0e-03)\tabularnewline
&IS& 2.03e+00 (1.8e-02)& 2.22e-01 (5.9e-03)& 2.16e+00 (1.9e-02)& \textbf{5.32e-01} (7.0e-03)\tabularnewline
&MONMLP (2x2)& 1.87e+00 (1.7e-02)& 2.96e-01 (6.2e-03)& 1.81e+00 (1.8e-02)& 7.30e-01 (1.0e-02)\tabularnewline
&MONMLP (4x2)& 1.87e+00 (1.7e-02)& 2.98e-01 (6.2e-03)& 1.71e+00 (1.8e-02)& 7.53e-01 (1.0e-02)\tabularnewline
&MONMLP (32x2)& 2.04e+00 (1.9e-02)& 2.57e-01 (5.6e-03)& 1.84e+00 (2.6e-02)& 9.35e-01 (1.7e-02)\tabularnewline
&MCB1& 2.01e+00 (1.8e-02)& \textbf{1.82e-01} (4.6e-03)& 2.21e+00 (2.0e-02)& 5.60e-01 (7.4e-03)\tabularnewline
&MCB2& 1.89e+00 (1.8e-02)& 2.30e-01 (5.6e-03)& 1.64e+00 (1.8e-02)& 5.99e-01 (7.9e-03)\tabularnewline
&CB1& 1.87e+00 (1.8e-02)& 6.07e+00 (5.7e+00)& 2.13e+00 (2.0e-02)& 6.07e-01 (8.0e-03)\tabularnewline
&CB2& 1.22e+00 (2.7e-02)& 4.31e+01 (9.8e+00)& 9.06e-01 (2.5e-02)& 7.42e+01 (1.5e+01)\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/2022-07-04T12_19_32+08_00_logit_and_growth.tex <==
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Noise} & \multirow{2}{*}{Method}&\multicolumn{2}{c}{Logistic Curve}&\multicolumn{2}{c}{Growth Curve}\tabularnewline
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&&MSFE&MSPE&MSFE&MSPE\tabularnewline
\midrule
\multirow{13}{*}{0.1}&MQB& 9.82e-03 (9.6e-05)& 2.56e-03 (4.4e-05)& 8.23e-03 (2.0e-04)& 1.19e-02 (2.3e-04)\tabularnewline
&QB& 8.64e-03 (8.4e-05)& 1.74e-03 (3.5e-05)& 4.31e-02 (1.8e-03)& 3.86e-02 (1.5e-03)\tabularnewline
&LOESS& 8.44e-03 (7.6e-05)& 1.50e-03 (2.8e-05)& 1.33e+00 (6.7e-03)& 8.61e-01 (5.0e-03)\tabularnewline
&Isotonic& 4.72e-03 (5.7e-05)& 2.92e-03 (3.5e-05)& 3.11e-04 (1.3e-05)& 2.19e-02 (4.0e-04)\tabularnewline
&SI& 8.51e-03 (7.6e-05)& \textbf{1.36e-03} (2.7e-05)& 1.33e+00 (6.7e-03)& 8.77e-01 (5.1e-03)\tabularnewline
&IS& 8.74e-03 (7.8e-05)& 1.51e-03 (2.8e-05)& 1.33e+00 (6.7e-03)& 8.61e-01 (5.0e-03)\tabularnewline
&MONMLP (2x2)& 6.94e-03 (6.9e-05)& 2.90e-03 (4.6e-05)& 9.34e-03 (9.8e-05)& \textbf{3.60e-03} (6.2e-05)\tabularnewline
&MONMLP (4x2)& 6.28e-03 (6.6e-05)& 3.33e-03 (4.6e-05)& 7.68e-03 (8.1e-05)& 5.12e-03 (4.0e-04)\tabularnewline
&MONMLP (32x2)& 6.19e-03 (7.0e-05)& 3.52e-03 (5.2e-05)& 8.70e-03 (6.6e-04)& 8.38e-03 (9.7e-04)\tabularnewline
&MCB1& 1.09e-02 (1.0e-04)& 2.78e-03 (3.0e-05)& 5.58e-03 (7.6e-05)& 5.66e-03 (6.9e-05)\tabularnewline
&MCB2& 6.66e-03 (8.2e-05)& 2.44e-03 (3.8e-05)& 1.41e-03 (3.7e-05)& 4.01e-02 (1.2e-03)\tabularnewline
&CB1& 8.98e-03 (8.6e-05)& 1.95e-03 (3.1e-05)& 5.48e-03 (7.6e-05)& 6.00e-03 (7.2e-05)\tabularnewline
&CB2& 4.03e-03 (1.1e-04)& 2.29e-01 (4.2e-02)& 3.75e-04 (3.1e-05)& 8.68e-01 (7.9e-02)\tabularnewline
\midrule
\multirow{13}{*}{1.0}&MQB& 9.53e-01 (8.3e-03)& 1.12e-01 (2.9e-03)& 1.33e+00 (2.2e-02)& 5.19e-01 (8.2e-03)\tabularnewline
&QB& 9.00e-01 (7.9e-03)& 1.03e-01 (2.4e-03)& 2.33e+00 (3.3e-02)& 1.23e+00 (1.9e-02)\tabularnewline
&LOESS& 8.16e-01 (7.4e-03)& 1.41e-01 (2.9e-03)& 2.14e+00 (1.5e-02)& 1.01e+00 (7.3e-03)\tabularnewline
&Isotonic& 7.60e-01 (7.3e-03)& 1.34e-01 (2.7e-03)& 3.69e-01 (4.9e-03)& 3.61e-01 (4.2e-03)\tabularnewline
&SI& 8.59e-01 (7.6e-03)& 9.68e-02 (2.1e-03)& 2.14e+00 (1.5e-02)& 1.03e+00 (7.5e-03)\tabularnewline
&IS& 8.86e-01 (7.9e-03)& 1.10e-01 (2.4e-03)& 2.16e+00 (1.5e-02)& 1.02e+00 (7.4e-03)\tabularnewline
&MONMLP (2x2)& 8.05e-01 (7.5e-03)& 1.42e-01 (2.9e-03)& 7.26e-01 (7.1e-03)& 3.37e-01 (9.8e-03)\tabularnewline
&MONMLP (4x2)& 8.04e-01 (7.5e-03)& 1.42e-01 (2.9e-03)& 6.42e-01 (6.9e-03)& 3.90e-01 (9.1e-03)\tabularnewline
&MONMLP (32x2)& 8.56e-01 (7.8e-03)& 1.12e-01 (2.6e-03)& 6.24e-01 (7.8e-03)& 4.15e-01 (1.0e-02)\tabularnewline
&MCB1& 8.89e-01 (7.8e-03)& \textbf{8.78e-02} (2.1e-03)& 8.00e-01 (8.8e-03)& \textbf{2.48e-01} (3.7e-03)\tabularnewline
&MCB2& 8.26e-01 (7.8e-03)& 1.13e-01 (2.5e-03)& 5.40e-01 (7.4e-03)& 3.50e-01 (5.1e-03)\tabularnewline
&CB1& 8.25e-01 (7.6e-03)& 1.55e-01 (3.7e-03)& 7.64e-01 (8.7e-03)& 3.06e-01 (4.3e-03)\tabularnewline
&CB2& 5.28e-01 (1.2e-02)& 2.24e+01 (3.6e+00)& 3.08e-01 (9.7e-03)& 1.88e+01 (2.9e+00)\tabularnewline
\midrule
\multirow{13}{*}{1.5}&MQB& 2.12e+00 (1.9e-02)& 2.24e-01 (6.6e-03)& 2.74e+00 (4.0e-02)& 9.26e-01 (1.6e-02)\tabularnewline
&QB& 1.99e+00 (1.8e-02)& 2.18e-01 (5.6e-03)& 3.77e+00 (4.1e-02)& 1.64e+00 (1.7e-02)\tabularnewline
&LOESS& 1.83e+00 (1.7e-02)& 3.08e-01 (6.2e-03)& 3.18e+00 (2.5e-02)& 1.19e+00 (1.1e-02)\tabularnewline
&Isotonic& 1.75e+00 (1.7e-02)& 2.84e-01 (6.2e-03)& 1.00e+00 (1.2e-02)& 6.88e-01 (8.2e-03)\tabularnewline
&SI& 1.94e+00 (1.8e-02)& 1.98e-01 (4.9e-03)& 3.19e+00 (2.5e-02)& 1.18e+00 (1.1e-02)\tabularnewline
&IS& 2.00e+00 (1.8e-02)& 2.41e-01 (5.7e-03)& 3.25e+00 (2.5e-02)& 1.18e+00 (1.1e-02)\tabularnewline
&MONMLP (2x2)& 1.84e+00 (1.7e-02)& 2.87e-01 (6.3e-03)& 1.62e+00 (1.6e-02)& 6.84e-01 (1.5e-02)\tabularnewline
&MONMLP (4x2)& 1.84e+00 (1.7e-02)& 2.84e-01 (6.4e-03)& 1.45e+00 (1.5e-02)& 8.09e-01 (1.6e-02)\tabularnewline
&MONMLP (32x2)& 1.94e+00 (1.8e-02)& 2.15e-01 (5.7e-03)& 1.43e+00 (1.6e-02)& 8.57e-01 (1.8e-02)\tabularnewline
&MCB1& 1.99e+00 (1.8e-02)& \textbf{1.79e-01} (4.6e-03)& 1.85e+00 (1.9e-02)& \textbf{4.83e-01} (7.5e-03)\tabularnewline
&MCB2& 1.87e+00 (1.8e-02)& 2.33e-01 (5.7e-03)& 1.36e+00 (1.7e-02)& 6.46e-01 (9.2e-03)\tabularnewline
&CB1& 1.84e+00 (1.7e-02)& 3.40e-01 (7.8e-03)& 1.76e+00 (1.9e-02)& 6.17e-01 (8.6e-03)\tabularnewline
&CB2& 1.19e+00 (2.6e-02)& 7.04e+01 (1.4e+01)& 7.95e-01 (2.3e-02)& 6.25e+01 (1.3e+01)\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/2023-01-17T17_20_41-05_00_cubic_and_steps.tex <==
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Noise $\sigma$} & \multirow{2}{*}{Method}&\multicolumn{2}{c}{Cubic Curve}&\multicolumn{2}{c}{Step Curve}\tabularnewline
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&&MSFE&MSPE&MSFE&MSPE\tabularnewline
\midrule
\multirow{15}{*}{0.1}&MQB& 8.85e-03 (2.8e-04)& 2.47e-03 (1.7e-04)& 1.34e-01 (7.2e-03)& 1.49e-01 (6.3e-03)\tabularnewline
&QB& 8.07e-03 (2.4e-04)& 1.65e-03 (1.1e-04)& 1.49e-01 (7.5e-03)& 1.64e-01 (6.9e-03)\tabularnewline
&LOESS& 8.61e-03 (2.4e-04)& 1.95e-03 (1.1e-04)& 2.33e-01 (8.0e-03)& 2.34e-01 (7.9e-03)\tabularnewline
&Isotonic& 3.72e-03 (1.6e-04)& 3.44e-03 (1.4e-04)& 4.93e-03 (2.1e-04)& \textbf{5.56e-02} (1.3e-03)\tabularnewline
&SI& 8.66e-03 (2.4e-04)& 1.92e-03 (1.2e-04)& 2.32e-01 (7.9e-03)& 2.34e-01 (7.8e-03)\tabularnewline
&IS& 8.97e-03 (2.5e-04)& 2.07e-03 (1.2e-04)& 2.34e-01 (8.1e-03)& 2.35e-01 (7.9e-03)\tabularnewline
&MONMLP (2x2)& 1.41e-02 (1.2e-03)& 7.83e-03 (9.5e-04)& 1.42e-01 (1.1e-02)& 1.61e-01 (1.0e-02)\tabularnewline
&MONMLP (4x2)& 1.26e-02 (1.1e-03)& 6.80e-03 (8.7e-04)& 1.08e-01 (9.0e-03)& 1.37e-01 (7.8e-03)\tabularnewline
&MONMLP (32x2)& 7.81e-03 (6.1e-04)& 4.56e-03 (5.2e-04)& 8.68e-02 (8.9e-03)& 1.39e-01 (7.9e-03)\tabularnewline
&MCS1& 8.26e-03 (2.4e-04)& \textbf{1.35e-03} (1.1e-04)& 2.32e-01 (1.3e-02)& 2.38e-01 (1.2e-02)\tabularnewline
&MCS2& 6.06e-03 (2.7e-04)& 2.72e-03 (1.6e-04)& 3.08e-02 (1.3e-03)& 6.73e-02 (1.4e-03)\tabularnewline
&CS1& 7.98e-03 (2.3e-04)& 1.58e-03 (1.1e-04)& 2.10e-01 (1.2e-02)& 2.19e-01 (1.1e-02)\tabularnewline
&CS2& 4.56e-03 (3.6e-04)& 9.04e-02 (3.6e-02)& 2.95e-03 (5.3e-04)& 1.20e+01 (5.6e+00)\tabularnewline
&MSS& 6.90e-03 (2.5e-04)& 2.20e-03 (1.5e-04)& 4.52e-02 (3.7e-03)& 7.51e-02 (2.8e-03)\tabularnewline
&SS& 5.98e-03 (3.3e-04)& 3.21e-03 (3.1e-04)& 3.32e-02 (4.3e-03)& 7.74e-02 (2.7e-03)\tabularnewline
\midrule
\multirow{15}{*}{1.0}&MQB& 9.69e-01 (2.8e-02)& 1.07e-01 (8.1e-03)& 1.21e+00 (4.3e-02)& 4.73e-01 (1.6e-02)\tabularnewline
&QB& 9.19e-01 (2.7e-02)& 1.14e-01 (7.7e-03)& 1.13e+00 (3.9e-02)& 4.42e-01 (1.5e-02)\tabularnewline
&LOESS& 8.43e-01 (2.6e-02)& 1.30e-01 (9.1e-03)& 1.05e+00 (3.3e-02)& 3.80e-01 (1.1e-02)\tabularnewline
&Isotonic& 7.39e-01 (2.5e-02)& 1.36e-01 (7.9e-03)& 5.24e-01 (2.1e-02)& 3.79e-01 (1.2e-02)\tabularnewline
&SI& 8.72e-01 (2.6e-02)& 9.57e-02 (6.7e-03)& 1.05e+00 (3.3e-02)& 3.77e-01 (1.1e-02)\tabularnewline
&IS& 8.98e-01 (2.7e-02)& 1.04e-01 (7.6e-03)& 1.08e+00 (3.4e-02)& 3.84e-01 (1.1e-02)\tabularnewline
&MONMLP (2x2)& 8.09e-01 (2.5e-02)& 1.59e-01 (8.7e-03)& 8.32e-01 (2.9e-02)& 4.31e-01 (1.5e-02)\tabularnewline
&MONMLP (4x2)& 8.03e-01 (2.6e-02)& 1.63e-01 (8.5e-03)& 7.78e-01 (2.9e-02)& 4.42e-01 (1.7e-02)\tabularnewline
&MONMLP (32x2)& 9.29e-01 (2.8e-02)& 1.57e-01 (7.8e-03)& 7.33e-01 (3.1e-02)& 4.89e-01 (2.0e-02)\tabularnewline
&MCS1& 8.91e-01 (2.7e-02)& 8.90e-02 (6.5e-03)& 1.10e+00 (3.6e-02)& 4.25e-01 (1.5e-02)\tabularnewline
&MCS2& 8.20e-01 (2.8e-02)& 1.14e-01 (7.3e-03)& 6.99e-01 (3.1e-02)& \textbf{3.73e-01} (1.2e-02)\tabularnewline
&CS1& 8.49e-01 (2.7e-02)& 1.40e-01 (1.0e-02)& 1.04e+00 (3.5e-02)& 4.24e-01 (1.3e-02)\tabularnewline
&CS2& 5.84e-01 (4.1e-02)& 2.79e+01 (1.2e+01)& 3.63e-01 (4.0e-02)& 3.60e+01 (1.9e+01)\tabularnewline
&MSS& 8.88e-01 (2.9e-02)& \textbf{8.76e-02} (6.2e-03)& 9.09e-01 (3.9e-02)& 3.74e-01 (1.2e-02)\tabularnewline
&SS& 7.69e-01 (4.1e-02)& 1.95e-01 (2.4e-02)& 8.12e-01 (4.8e-02)& 4.62e-01 (2.6e-02)\tabularnewline
\midrule
\multirow{15}{*}{1.5}&MQB& 2.22e+00 (6.4e-02)& 2.47e-01 (2.3e-02)& 2.53e+00 (7.9e-02)& 7.33e-01 (3.4e-02)\tabularnewline
&QB& 2.10e+00 (6.3e-02)& 2.28e-01 (1.7e-02)& 2.38e+00 (7.5e-02)& 6.32e-01 (2.8e-02)\tabularnewline
&LOESS& 1.92e+00 (6.1e-02)& 2.94e-01 (1.8e-02)& 2.15e+00 (6.5e-02)& 5.38e-01 (2.2e-02)\tabularnewline
&Isotonic& 1.76e+00 (5.6e-02)& 2.86e-01 (1.8e-02)& 1.31e+00 (5.0e-02)& 6.24e-01 (2.4e-02)\tabularnewline
&SI& 2.02e+00 (6.2e-02)& 1.91e-01 (1.4e-02)& 2.16e+00 (6.6e-02)& \textbf{5.29e-01} (2.2e-02)\tabularnewline
&IS& 2.07e+00 (6.3e-02)& 2.25e-01 (1.6e-02)& 2.22e+00 (6.8e-02)& 5.43e-01 (2.2e-02)\tabularnewline
&MONMLP (2x2)& 1.90e+00 (5.8e-02)& 3.04e-01 (1.9e-02)& 1.86e+00 (6.4e-02)& 7.14e-01 (2.7e-02)\tabularnewline
&MONMLP (4x2)& 1.89e+00 (6.2e-02)& 3.11e-01 (2.0e-02)& 1.73e+00 (6.3e-02)& 7.60e-01 (3.2e-02)\tabularnewline
&MONMLP (32x2)& 2.09e+00 (6.4e-02)& 2.57e-01 (1.6e-02)& 1.90e+00 (9.8e-02)& 9.28e-01 (6.0e-02)\tabularnewline
&MCS1& 2.05e+00 (6.1e-02)& 1.86e-01 (1.4e-02)& 2.27e+00 (6.9e-02)& 5.64e-01 (2.4e-02)\tabularnewline
&MCS2& 1.91e+00 (6.2e-02)& 2.39e-01 (1.7e-02)& 1.66e+00 (5.9e-02)& 5.83e-01 (2.4e-02)\tabularnewline
&CS1& 1.92e+00 (6.2e-02)& 3.37e-01 (2.1e-02)& 2.20e+00 (7.0e-02)& 6.07e-01 (2.5e-02)\tabularnewline
&CS2& 1.34e+00 (9.3e-02)& 1.48e+01 (6.1e+00)& 8.27e-01 (7.7e-02)& 3.74e+01 (2.0e+01)\tabularnewline
&MSS& 2.05e+00 (6.5e-02)& \textbf{1.80e-01} (1.4e-02)& 1.98e+00 (7.5e-02)& 5.70e-01 (2.4e-02)\tabularnewline
&SS& 1.73e+00 (9.8e-02)& 5.01e-01 (6.7e-02)& 1.64e+00 (1.1e-01)& 8.87e-01 (7.1e-02)\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/2023-01-17T17_20_41-05_00_logit_and_growth.tex <==
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Noise $\sigma$} & \multirow{2}{*}{Method}&\multicolumn{2}{c}{Logistic Curve}&\multicolumn{2}{c}{Growth Curve}\tabularnewline
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&&MSFE&MSPE&MSFE&MSPE\tabularnewline
\midrule
\multirow{15}{*}{0.1}&MQB& 9.78e-03 (3.2e-04)& 2.68e-03 (1.4e-04)& 9.01e-03 (1.1e-03)& 1.10e-02 (9.6e-04)\tabularnewline
&QB& 8.65e-03 (2.8e-04)& 1.65e-03 (8.8e-05)& 5.22e-02 (5.6e-03)& 4.39e-02 (4.0e-03)\tabularnewline
&LOESS& 8.37e-03 (2.5e-04)& 1.53e-03 (8.9e-05)& 1.32e+00 (2.0e-02)& 8.61e-01 (1.5e-02)\tabularnewline
&Isotonic& 4.55e-03 (1.8e-04)& 3.00e-03 (1.1e-04)& 3.23e-04 (3.8e-05)& 2.09e-02 (1.2e-03)\tabularnewline
&SI& 8.44e-03 (2.5e-04)& \textbf{1.44e-03} (8.9e-05)& 1.32e+00 (2.0e-02)& 8.77e-01 (1.6e-02)\tabularnewline
&IS& 8.64e-03 (2.6e-04)& 1.55e-03 (9.3e-05)& 1.32e+00 (2.0e-02)& 8.60e-01 (1.5e-02)\tabularnewline
&MONMLP (2x2)& 6.78e-03 (2.3e-04)& 3.02e-03 (1.5e-04)& 8.91e-03 (3.1e-04)& \textbf{3.50e-03} (2.7e-04)\tabularnewline
&MONMLP (4x2)& 6.19e-03 (2.3e-04)& 3.32e-03 (1.6e-04)& 7.35e-03 (2.8e-04)& 7.22e-03 (1.7e-03)\tabularnewline
&MONMLP (32x2)& 6.06e-03 (2.5e-04)& 3.59e-03 (1.8e-04)& 1.01e-02 (3.2e-03)& 1.30e-02 (4.5e-03)\tabularnewline
&MCS1& 1.04e-02 (3.3e-04)& 2.65e-03 (1.0e-04)& 5.24e-03 (2.4e-04)& 5.24e-03 (2.2e-04)\tabularnewline
&MCS2& 6.49e-03 (2.6e-04)& 2.53e-03 (1.3e-04)& 1.46e-03 (1.2e-04)& 3.96e-02 (3.0e-03)\tabularnewline
&CS1& 8.77e-03 (2.7e-04)& 1.88e-03 (9.2e-05)& 5.14e-03 (2.5e-04)& 5.59e-03 (2.5e-04)\tabularnewline
&CS2& 3.80e-03 (3.4e-04)& 1.00e-01 (4.4e-02)& 3.66e-04 (9.2e-05)& 9.96e-01 (2.1e-01)\tabularnewline
&MSS& 7.31e-03 (2.8e-04)& 1.97e-03 (1.1e-04)& 1.21e-03 (1.1e-04)& 2.52e-02 (3.3e-03)\tabularnewline
&SS& 6.31e-03 (3.6e-04)& 2.96e-03 (2.8e-04)& 2.14e-04 (8.4e-05)& 1.23e-02 (4.9e-04)\tabularnewline
\midrule
\multirow{15}{*}{1.0}&MQB& 9.73e-01 (2.7e-02)& 1.26e-01 (1.4e-02)& 1.37e+00 (6.9e-02)& 5.47e-01 (2.8e-02)\tabularnewline
&QB& 9.13e-01 (2.6e-02)& 1.05e-01 (9.5e-03)& 2.47e+00 (1.0e-01)& 1.26e+00 (5.9e-02)\tabularnewline
&LOESS& 8.35e-01 (2.5e-02)& 1.41e-01 (1.0e-02)& 2.15e+00 (4.4e-02)& 9.76e-01 (2.3e-02)\tabularnewline
&Isotonic& 7.63e-01 (2.5e-02)& 1.44e-01 (8.8e-03)& 3.77e-01 (1.8e-02)& 3.57e-01 (1.3e-02)\tabularnewline
&SI& 8.71e-01 (2.6e-02)& 1.04e-01 (8.6e-03)& 2.15e+00 (4.4e-02)& 9.88e-01 (2.4e-02)\tabularnewline
&IS& 9.01e-01 (2.7e-02)& 1.19e-01 (8.6e-03)& 2.17e+00 (4.4e-02)& 9.82e-01 (2.3e-02)\tabularnewline
&MONMLP (2x2)& 8.10e-01 (2.5e-02)& 1.53e-01 (9.8e-03)& 7.30e-01 (2.7e-02)& 3.93e-01 (3.6e-02)\tabularnewline
&MONMLP (4x2)& 8.11e-01 (2.6e-02)& 1.47e-01 (9.3e-03)& 6.31e-01 (2.5e-02)& 4.44e-01 (3.6e-02)\tabularnewline
&MONMLP (32x2)& 8.67e-01 (2.7e-02)& 1.18e-01 (9.4e-03)& 6.17e-01 (2.7e-02)& 4.67e-01 (4.4e-02)\tabularnewline
&MCS1& 9.04e-01 (2.7e-02)& \textbf{9.06e-02} (8.1e-03)& 8.01e-01 (3.2e-02)& \textbf{2.58e-01} (1.1e-02)\tabularnewline
&MCS2& 8.22e-01 (2.7e-02)& 1.23e-01 (8.8e-03)& 5.47e-01 (2.6e-02)& 3.63e-01 (1.8e-02)\tabularnewline
&CS1& 8.49e-01 (2.6e-02)& 1.48e-01 (1.1e-02)& 7.60e-01 (3.2e-02)& 3.21e-01 (1.5e-02)\tabularnewline
&CS2& 4.96e-01 (3.9e-02)& 1.68e+01 (6.5e+00)& 3.20e-01 (3.1e-02)& 5.84e+01 (5.0e+01)\tabularnewline
&MSS& 8.86e-01 (2.8e-02)& 9.13e-02 (8.6e-03)& 6.31e-01 (3.2e-02)& 3.28e-01 (1.5e-02)\tabularnewline
&SS& 7.57e-01 (4.0e-02)& 2.15e-01 (3.0e-02)& 4.94e-01 (3.7e-02)& 4.60e-01 (2.5e-02)\tabularnewline
\midrule
\multirow{15}{*}{1.5}&MQB& 2.13e+00 (5.6e-02)& 2.11e-01 (2.3e-02)& 2.51e+00 (1.1e-01)& 8.78e-01 (4.9e-02)\tabularnewline
&QB& 2.00e+00 (5.2e-02)& 2.20e-01 (1.9e-02)& 3.69e+00 (1.1e-01)& 1.75e+00 (5.0e-02)\tabularnewline
&LOESS& 1.81e+00 (5.1e-02)& 3.14e-01 (2.1e-02)& 2.94e+00 (7.1e-02)& 1.20e+00 (3.2e-02)\tabularnewline
&Isotonic& 1.74e+00 (5.2e-02)& 2.84e-01 (1.9e-02)& 9.20e-01 (3.8e-02)& 6.49e-01 (2.6e-02)\tabularnewline
&SI& 1.94e+00 (5.4e-02)& 1.94e-01 (1.5e-02)& 2.94e+00 (7.1e-02)& 1.19e+00 (3.2e-02)\tabularnewline
&IS& 1.99e+00 (5.5e-02)& 2.36e-01 (1.7e-02)& 3.00e+00 (7.2e-02)& 1.18e+00 (3.2e-02)\tabularnewline
&MONMLP (2x2)& 1.84e+00 (5.4e-02)& 2.88e-01 (2.0e-02)& 1.48e+00 (4.9e-02)& 6.72e-01 (4.9e-02)\tabularnewline
&MONMLP (4x2)& 1.83e+00 (5.3e-02)& 2.90e-01 (2.0e-02)& 1.33e+00 (4.5e-02)& 7.54e-01 (4.8e-02)\tabularnewline
&MONMLP (32x2)& 1.93e+00 (5.4e-02)& 2.14e-01 (1.8e-02)& 1.30e+00 (4.7e-02)& 8.09e-01 (5.6e-02)\tabularnewline
&MCS1& 1.99e+00 (5.4e-02)& 1.77e-01 (1.5e-02)& 1.73e+00 (6.0e-02)& \textbf{4.82e-01} (2.4e-02)\tabularnewline
&MCS2& 1.86e+00 (5.4e-02)& 2.39e-01 (1.9e-02)& 1.27e+00 (5.0e-02)& 5.89e-01 (2.7e-02)\tabularnewline
&CS1& 1.83e+00 (5.1e-02)& 3.44e-01 (2.6e-02)& 1.65e+00 (5.7e-02)& 5.94e-01 (2.8e-02)\tabularnewline
&CS2& 1.15e+00 (7.9e-02)& 2.86e+01 (1.3e+01)& 8.21e-01 (6.6e-02)& 1.35e+01 (6.8e+00)\tabularnewline
&MSS& 1.96e+00 (5.5e-02)& \textbf{1.74e-01} (1.5e-02)& 1.44e+00 (6.2e-02)& 6.02e-01 (2.9e-02)\tabularnewline
&SS& 1.64e+00 (8.3e-02)& 4.85e-01 (7.3e-02)& 1.11e+00 (8.1e-02)& 9.50e-01 (6.0e-02)\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/cmpr_logit_growth.tex <==
\begin{tabular}{lllll}
\hline
\toprule
 & \multicolumn{2}{c}{Logistic Curve} & \multicolumn{2}{c}{Growth Curve} \\ 
\cmidrule(lr){2-3}\cmidrule{4-5}
 & \multicolumn{1}{c}{RMSE} & \multicolumn{1}{c}{RMSE(3)} & \multicolumn{1}{c}{RMSE} & \multicolumn{1}{c}{RMSE(3)} \\ 
\midrule
MQB0 & 0.0398 (0.0005) & 0.0411 (0.0005) & 0.8183 (0.0106) & 0.5964 (0.0070)\\ 
MQB & 4.90e-02 (4.7e-04) & 4.62e-02 (4.8e-04) & 8.72e-01 (9.6e-03) & 6.77e-01 (7.5e-03)\\ 
QB & 4.35e-02 (4.4e-04) & 4.00e-02 (4.6e-04) & 1.04e+00 (1.1e-02) & 8.46e-01 (9.7e-03)\\ 
LOESS & 3.84e-02 (3.7e-04) & 3.46e-02 (3.9e-04) & 9.14e-01 (8.5e-03) & 7.09e-01 (7.9e-03)\\ 
SI & 3.60e-02 (3.7e-04) & 3.42e-02 (3.9e-04) & 9.01e-01 (8.5e-03) & 7.01e-01 (7.9e-03)\\ 
IS & 3.76e-02 (3.7e-04) & 3.45e-02 (3.9e-04) & 9.00e-01 (8.7e-03) & 6.95e-01 (8.0e-03)\\ 
MCB1 & 4.58e-02 (3.8e-04) & 4.36e-02 (4.1e-04) & 6.47e-01 (5.9e-03) & 5.39e-01 (5.9e-03)\\ 
MCB2 & 4.76e-02 (4.3e-04) & 4.56e-02 (4.4e-04) & 7.42e-01 (6.2e-03) & 6.51e-01 (6.5e-03)\\ 
CB1 & 4.34e-02 (3.6e-04) & 3.92e-02 (3.9e-04) & 7.22e-01 (6.3e-03) & 6.22e-01 (6.6e-03)\\ 
CB2 & 7.10e-02 (7.9e-04) & 6.82e-02 (8.5e-04) & 1.09e+00 (1.1e-02) & 1.03e+00 (1.2e-02)\\ 
\bottomrule
\end{tabular}

==> res/mono_fit/erf_2023-09-25T17_54_13-04_00_nrep100.tex <==
\begin{tabular}{ccccc}
\toprule
Noise $\sigma$ & Method&$\frac 1n L_1$&$\frac{1}{\sqrt n}L_2$&$L_\infty$\tabularnewline
\midrule
\multirow{14}{*}{0.15}&Cubic Spline (CS)& 9.71e-02 (1.6e-03)\textsuperscript{7}& 1.22e-01 (1.9e-03)\textsuperscript{6}& 3.46e-01 (5.9e-03)\textsuperscript{6}\tabularnewline
&Monotone CS (MCS)& 5.45e-02 (9.2e-04)\textsuperscript{3}& 7.22e-02 (1.1e-03)\textsuperscript{3}& \textbf{2.42e-01} (6.3e-03)\textsuperscript{1}\tabularnewline
&Smoothing Spline (SS)& 6.27e-02 (8.1e-04)\textsuperscript{5}& 8.02e-02 (1.0e-03)\textsuperscript{4}& 2.58e-01 (7.3e-03)\textsuperscript{3}\tabularnewline
&Montone SS (MSS)& \textbf{5.21e-02} (8.8e-04)\textsuperscript{1}& \textbf{7.05e-02} (1.2e-03)\textsuperscript{1}& 2.55e-01 (7.5e-03)\textsuperscript{2}\tabularnewline
&Quadratic Spline (QS)& 1.22e-01 (2.8e-03)\textsuperscript{9}& 1.64e-01 (3.7e-03)\textsuperscript{9}& 5.45e-01 (1.5e-02)\textsuperscript{8}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 9.53e-02 (1.8e-03)\textsuperscript{6}& 1.46e-01 (3.1e-03)\textsuperscript{7}& 6.02e-01 (1.9e-02)\textsuperscript{9}\tabularnewline
&LOESS& 2.96e-01 (2.1e-03)\textsuperscript{10}& 3.54e-01 (2.2e-03)\textsuperscript{10}& 7.79e-01 (5.7e-03)\textsuperscript{10}\tabularnewline
&Isotonic& 6.24e-02 (9.2e-04)\textsuperscript{4}& 8.39e-02 (1.0e-03)\textsuperscript{5}& 2.92e-01 (6.6e-03)\textsuperscript{5}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 2.96e-01 (2.1e-03)\textsuperscript{11}& 3.54e-01 (2.2e-03)\textsuperscript{11}& 7.79e-01 (5.7e-03)\textsuperscript{11}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 2.97e-01 (2.1e-03)\textsuperscript{12}& 3.54e-01 (2.2e-03)\textsuperscript{12}& 7.79e-01 (5.6e-03)\textsuperscript{12}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 3.28e-01 (2.3e-03)\textsuperscript{13}& 3.91e-01 (2.3e-03)\textsuperscript{13}& 8.53e-01 (6.9e-03)\textsuperscript{13}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 1.11e-01 (8.3e-03)\textsuperscript{8}& 1.49e-01 (1.1e-02)\textsuperscript{8}& 4.42e-01 (2.5e-02)\textsuperscript{7}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 5.29e-02 (7.9e-04)\textsuperscript{2}& 7.20e-02 (1.1e-03)\textsuperscript{2}& 2.62e-01 (8.0e-03)\textsuperscript{4}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 3.33e-01 (2.3e-03)\textsuperscript{14}& 4.05e-01 (2.6e-03)\textsuperscript{14}& 1.03e+00 (1.3e-02)\textsuperscript{14}\tabularnewline
\midrule
\multirow{14}{*}{0.3}&Cubic Spline (CS)& 1.86e-01 (3.8e-03)\textsuperscript{9}& 2.35e-01 (4.7e-03)\textsuperscript{9}& 6.90e-01 (1.7e-02)\textsuperscript{9}\tabularnewline
&Monotone CS (MCS)& 1.00e-01 (1.9e-03)\textsuperscript{3}& 1.32e-01 (2.1e-03)\textsuperscript{3}& 4.39e-01 (1.4e-02)\textsuperscript{4}\tabularnewline
&Smoothing Spline (SS)& 1.12e-01 (1.7e-03)\textsuperscript{5}& 1.41e-01 (2.0e-03)\textsuperscript{4}& 4.16e-01 (1.1e-02)\textsuperscript{2}\tabularnewline
&Montone SS (MSS)& \textbf{9.86e-02} (1.8e-03)\textsuperscript{1}& \textbf{1.28e-01} (2.0e-03)\textsuperscript{1}& \textbf{4.08e-01} (1.1e-02)\textsuperscript{1}\tabularnewline
&Quadratic Spline (QS)& 1.72e-01 (3.8e-03)\textsuperscript{8}& 2.23e-01 (4.9e-03)\textsuperscript{8}& 6.53e-01 (1.7e-02)\textsuperscript{8}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 1.49e-01 (2.9e-03)\textsuperscript{6}& 2.00e-01 (3.6e-03)\textsuperscript{6}& 6.51e-01 (1.7e-02)\textsuperscript{7}\tabularnewline
&LOESS& 2.97e-01 (1.8e-03)\textsuperscript{10}& 3.57e-01 (1.8e-03)\textsuperscript{10}& 7.90e-01 (6.3e-03)\textsuperscript{11}\tabularnewline
&Isotonic& 1.11e-01 (1.8e-03)\textsuperscript{4}& 1.49e-01 (2.0e-03)\textsuperscript{5}& 5.07e-01 (1.4e-02)\textsuperscript{5}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 2.97e-01 (1.8e-03)\textsuperscript{11}& 3.57e-01 (1.8e-03)\textsuperscript{11}& 7.90e-01 (6.3e-03)\textsuperscript{12}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 2.98e-01 (1.8e-03)\textsuperscript{12}& 3.58e-01 (1.8e-03)\textsuperscript{12}& 7.89e-01 (6.2e-03)\textsuperscript{10}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 3.26e-01 (2.2e-03)\textsuperscript{13}& 3.91e-01 (2.1e-03)\textsuperscript{13}& 8.77e-01 (7.7e-03)\textsuperscript{13}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 1.63e-01 (8.0e-03)\textsuperscript{7}& 2.10e-01 (9.6e-03)\textsuperscript{7}& 6.02e-01 (2.2e-02)\textsuperscript{6}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 9.87e-02 (1.9e-03)\textsuperscript{2}& 1.29e-01 (2.1e-03)\textsuperscript{2}& 4.16e-01 (1.1e-02)\textsuperscript{3}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 3.36e-01 (3.3e-03)\textsuperscript{14}& 4.12e-01 (4.1e-03)\textsuperscript{14}& 1.06e+00 (1.9e-02)\textsuperscript{14}\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/growth_2023-09-25T17_54_13-04_00_nrep100.tex <==
\begin{tabular}{ccccc}
\toprule
Noise $\sigma$ & Method&$\frac 1n L_1$&$\frac{1}{\sqrt n}L_2$&$L_\infty$\tabularnewline
\midrule
\multirow{14}{*}{0.1}&Cubic Spline (CS)& 5.97e-02 (2.0e-03)\textsuperscript{7}& 7.50e-02 (2.4e-03)\textsuperscript{7}& 2.10e-01 (7.5e-03)\textsuperscript{6}\tabularnewline
&Monotone CS (MCS)& 4.71e-02 (1.1e-03)\textsuperscript{6}& 5.97e-02 (1.4e-03)\textsuperscript{5}& 1.76e-01 (5.8e-03)\textsuperscript{2}\tabularnewline
&Smoothing Spline (SS)& 4.57e-02 (6.7e-04)\textsuperscript{4}& 5.90e-02 (7.9e-04)\textsuperscript{4}& 2.06e-01 (6.3e-03)\textsuperscript{5}\tabularnewline
&Montone SS (MSS)& 4.41e-02 (6.2e-04)\textsuperscript{3}& 5.70e-02 (7.5e-04)\textsuperscript{3}& 2.02e-01 (6.5e-03)\textsuperscript{4}\tabularnewline
&Quadratic Spline (QS)& 7.56e-02 (3.5e-03)\textsuperscript{9}& 1.37e-01 (7.2e-03)\textsuperscript{9}& 6.94e-01 (4.4e-02)\textsuperscript{9}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 4.64e-02 (9.7e-04)\textsuperscript{5}& 6.86e-02 (2.3e-03)\textsuperscript{6}& 3.31e-01 (2.4e-02)\textsuperscript{8}\tabularnewline
&LOESS& 4.19e-01 (9.4e-03)\textsuperscript{12}& 8.88e-01 (1.7e-02)\textsuperscript{10}& 4.88e+00 (1.2e-01)\textsuperscript{10}\tabularnewline
&Isotonic& 6.04e-02 (6.0e-04)\textsuperscript{8}& 7.69e-02 (7.7e-04)\textsuperscript{8}& 2.31e-01 (4.5e-03)\textsuperscript{7}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 4.19e-01 (9.4e-03)\textsuperscript{13}& 8.88e-01 (1.7e-02)\textsuperscript{11}& 4.88e+00 (1.2e-01)\textsuperscript{11}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 4.19e-01 (9.4e-03)\textsuperscript{11}& 8.88e-01 (1.7e-02)\textsuperscript{12}& 4.88e+00 (1.2e-01)\textsuperscript{12}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 7.07e-01 (1.2e-02)\textsuperscript{14}& 1.03e+00 (2.0e-02)\textsuperscript{14}& 5.21e+00 (1.2e-01)\textsuperscript{13}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& \textbf{2.68e-02} (6.3e-04)\textsuperscript{1}& \textbf{3.55e-02} (7.7e-04)\textsuperscript{1}& \textbf{1.32e-01} (5.0e-03)\textsuperscript{1}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 4.35e-02 (6.1e-04)\textsuperscript{2}& 5.60e-02 (7.3e-04)\textsuperscript{2}& 1.90e-01 (5.8e-03)\textsuperscript{3}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 2.98e-01 (8.6e-03)\textsuperscript{10}& 9.72e-01 (3.1e-02)\textsuperscript{13}& 6.21e+00 (1.9e-01)\textsuperscript{14}\tabularnewline
\midrule
\multirow{14}{*}{1.0}&Cubic Spline (CS)& 4.63e-01 (1.9e-02)\textsuperscript{9}& 5.83e-01 (2.4e-02)\textsuperscript{8}& 1.65e+00 (7.2e-02)\textsuperscript{7}\tabularnewline
&Monotone CS (MCS)& 2.83e-01 (6.4e-03)\textsuperscript{4}& 3.66e-01 (8.4e-03)\textsuperscript{4}& 1.20e+00 (4.5e-02)\textsuperscript{2}\tabularnewline
&Smoothing Spline (SS)& 2.86e-01 (5.5e-03)\textsuperscript{5}& 3.76e-01 (6.8e-03)\textsuperscript{5}& 1.34e+00 (5.1e-02)\textsuperscript{5}\tabularnewline
&Montone SS (MSS)& 2.55e-01 (4.4e-03)\textsuperscript{3}& 3.39e-01 (6.1e-03)\textsuperscript{3}& 1.31e+00 (5.3e-02)\textsuperscript{4}\tabularnewline
&Quadratic Spline (QS)& 4.91e-01 (1.6e-02)\textsuperscript{10}& 7.40e-01 (2.3e-02)\textsuperscript{9}& 3.64e+00 (1.3e-01)\textsuperscript{9}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 2.95e-01 (7.1e-03)\textsuperscript{6}& 4.22e-01 (1.1e-02)\textsuperscript{6}& 1.84e+00 (1.0e-01)\textsuperscript{8}\tabularnewline
&LOESS& 5.08e-01 (9.2e-03)\textsuperscript{12}& 9.37e-01 (1.5e-02)\textsuperscript{11}& 5.02e+00 (1.1e-01)\textsuperscript{11}\tabularnewline
&Isotonic& 3.47e-01 (4.6e-03)\textsuperscript{7}& 4.61e-01 (6.2e-03)\textsuperscript{7}& 1.60e+00 (3.9e-02)\textsuperscript{6}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 5.08e-01 (9.2e-03)\textsuperscript{11}& 9.37e-01 (1.5e-02)\textsuperscript{10}& 5.02e+00 (1.1e-01)\textsuperscript{12}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 5.09e-01 (8.9e-03)\textsuperscript{13}& 9.39e-01 (1.5e-02)\textsuperscript{12}& 5.01e+00 (1.1e-01)\textsuperscript{10}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 7.21e-01 (1.1e-02)\textsuperscript{14}& 1.06e+00 (1.8e-02)\textsuperscript{14}& 5.38e+00 (1.2e-01)\textsuperscript{13}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& \textbf{2.32e-01} (7.6e-03)\textsuperscript{1}& \textbf{3.05e-01} (9.9e-03)\textsuperscript{1}& \textbf{1.01e+00} (4.4e-02)\textsuperscript{1}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 2.54e-01 (4.5e-03)\textsuperscript{2}& 3.38e-01 (6.2e-03)\textsuperscript{2}& 1.29e+00 (5.3e-02)\textsuperscript{3}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 4.56e-01 (1.0e-02)\textsuperscript{8}& 1.05e+00 (3.0e-02)\textsuperscript{13}& 6.40e+00 (1.8e-01)\textsuperscript{14}\tabularnewline
\midrule
\multirow{14}{*}{1.5}&Cubic Spline (CS)& 6.67e-01 (3.1e-02)\textsuperscript{12}& 8.41e-01 (3.8e-02)\textsuperscript{8}& 2.37e+00 (1.0e-01)\textsuperscript{8}\tabularnewline
&Monotone CS (MCS)& 3.95e-01 (9.8e-03)\textsuperscript{4}& 5.18e-01 (1.3e-02)\textsuperscript{4}& 1.69e+00 (6.5e-02)\textsuperscript{2}\tabularnewline
&Smoothing Spline (SS)& 3.99e-01 (8.9e-03)\textsuperscript{5}& 5.30e-01 (1.0e-02)\textsuperscript{5}& 1.92e+00 (7.5e-02)\textsuperscript{5}\tabularnewline
&Montone SS (MSS)& 3.61e-01 (8.0e-03)\textsuperscript{3}& 4.84e-01 (9.7e-03)\textsuperscript{3}& 1.84e+00 (7.8e-02)\textsuperscript{4}\tabularnewline
&Quadratic Spline (QS)& 6.95e-01 (2.0e-02)\textsuperscript{13}& 9.80e-01 (2.9e-02)\textsuperscript{12}& 4.42e+00 (1.7e-01)\textsuperscript{9}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 4.09e-01 (1.2e-02)\textsuperscript{6}& 5.83e-01 (1.6e-02)\textsuperscript{6}& 2.37e+00 (1.4e-01)\textsuperscript{7}\tabularnewline
&LOESS& 5.75e-01 (1.2e-02)\textsuperscript{10}& 9.69e-01 (1.8e-02)\textsuperscript{10}& 4.85e+00 (1.3e-01)\textsuperscript{11}\tabularnewline
&Isotonic& 4.70e-01 (7.2e-03)\textsuperscript{7}& 6.33e-01 (9.5e-03)\textsuperscript{7}& 2.29e+00 (6.7e-02)\textsuperscript{6}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 5.74e-01 (1.2e-02)\textsuperscript{9}& 9.68e-01 (1.8e-02)\textsuperscript{9}& 4.85e+00 (1.3e-01)\textsuperscript{12}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 5.77e-01 (1.2e-02)\textsuperscript{11}& 9.74e-01 (1.8e-02)\textsuperscript{11}& 4.83e+00 (1.3e-01)\textsuperscript{10}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 7.46e-01 (1.2e-02)\textsuperscript{14}& 1.10e+00 (1.9e-02)\textsuperscript{14}& 5.26e+00 (1.3e-01)\textsuperscript{13}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& \textbf{3.43e-01} (1.0e-02)\textsuperscript{1}& \textbf{4.47e-01} (1.3e-02)\textsuperscript{1}& \textbf{1.41e+00} (6.1e-02)\textsuperscript{1}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 3.60e-01 (8.0e-03)\textsuperscript{2}& 4.81e-01 (9.8e-03)\textsuperscript{2}& 1.81e+00 (7.6e-02)\textsuperscript{3}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 5.19e-01 (1.3e-02)\textsuperscript{8}& 1.03e+00 (3.0e-02)\textsuperscript{13}& 6.03e+00 (2.0e-01)\textsuperscript{14}\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/logit_2023-09-25T17_54_13-04_00_nrep100.tex <==
\begin{tabular}{ccccc}
\toprule
Noise $\sigma$ & Method&$\frac 1n L_1$&$\frac{1}{\sqrt n}L_2$&$L_\infty$\tabularnewline
\midrule
\multirow{14}{*}{0.1}&Cubic Spline (CS)& 3.95e-02 (2.4e-03)\textsuperscript{13}& 4.97e-02 (3.0e-03)\textsuperscript{13}& 1.33e-01 (8.5e-03)\textsuperscript{13}\tabularnewline
&Monotone CS (MCS)& 2.34e-02 (8.1e-04)\textsuperscript{10}& 2.94e-02 (1.0e-03)\textsuperscript{10}& 7.98e-02 (4.8e-03)\textsuperscript{10}\tabularnewline
&Smoothing Spline (SS)& 1.89e-02 (6.3e-04)\textsuperscript{5}& 2.30e-02 (7.8e-04)\textsuperscript{5}& 5.13e-02 (2.2e-03)\textsuperscript{4}\tabularnewline
&Montone SS (MSS)& 1.80e-02 (5.8e-04)\textsuperscript{2}& 2.19e-02 (7.0e-04)\textsuperscript{2}& 4.75e-02 (1.9e-03)\textsuperscript{2}\tabularnewline
&Quadratic Spline (QS)& 2.17e-02 (6.3e-04)\textsuperscript{6}& 2.62e-02 (7.7e-04)\textsuperscript{6}& 6.07e-02 (2.7e-03)\textsuperscript{7}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 2.43e-02 (8.0e-04)\textsuperscript{11}& 2.90e-02 (9.2e-04)\textsuperscript{9}& 5.95e-02 (2.5e-03)\textsuperscript{6}\tabularnewline
&LOESS& 1.81e-02 (5.2e-04)\textsuperscript{3}& 2.24e-02 (6.2e-04)\textsuperscript{3}& 5.28e-02 (1.9e-03)\textsuperscript{5}\tabularnewline
&Isotonic& 2.97e-02 (5.5e-04)\textsuperscript{12}& 3.86e-02 (5.9e-04)\textsuperscript{12}& 1.24e-01 (3.6e-03)\textsuperscript{12}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& \textbf{1.72e-02} (5.5e-04)\textsuperscript{1}& \textbf{2.09e-02} (6.6e-04)\textsuperscript{1}& \textbf{4.22e-02} (1.4e-03)\textsuperscript{1}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 1.87e-02 (5.9e-04)\textsuperscript{4}& 2.29e-02 (7.0e-04)\textsuperscript{4}& 4.78e-02 (1.6e-03)\textsuperscript{3}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 7.73e-02 (4.3e-04)\textsuperscript{14}& 8.84e-02 (3.9e-04)\textsuperscript{14}& 1.80e-01 (2.7e-03)\textsuperscript{14}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 2.33e-02 (7.3e-04)\textsuperscript{9}& 3.00e-02 (9.1e-04)\textsuperscript{11}& 8.36e-02 (4.1e-03)\textsuperscript{11}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 2.30e-02 (5.6e-04)\textsuperscript{8}& 2.88e-02 (6.2e-04)\textsuperscript{8}& 7.34e-02 (2.0e-03)\textsuperscript{9}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 2.28e-02 (7.6e-04)\textsuperscript{7}& 2.82e-02 (9.1e-04)\textsuperscript{7}& 6.86e-02 (2.6e-03)\textsuperscript{8}\tabularnewline
\midrule
\multirow{14}{*}{1.0}&Cubic Spline (CS)& 3.69e-01 (2.2e-02)\textsuperscript{14}& 4.65e-01 (2.8e-02)\textsuperscript{14}& 1.36e+00 (9.0e-02)\textsuperscript{14}\tabularnewline
&Monotone CS (MCS)& 1.76e-01 (6.0e-03)\textsuperscript{10}& 2.27e-01 (8.3e-03)\textsuperscript{11}& 6.92e-01 (5.0e-02)\textsuperscript{12}\tabularnewline
&Smoothing Spline (SS)& 1.66e-01 (7.1e-03)\textsuperscript{6}& 2.05e-01 (8.8e-03)\textsuperscript{6}& 4.65e-01 (2.8e-02)\textsuperscript{6}\tabularnewline
&Montone SS (MSS)& \textbf{1.46e-01} (5.5e-03)\textsuperscript{1}& \textbf{1.78e-01} (6.3e-03)\textsuperscript{1}& \textbf{3.90e-01} (2.1e-02)\textsuperscript{1}\tabularnewline
&Quadratic Spline (QS)& 1.59e-01 (5.8e-03)\textsuperscript{4}& 1.96e-01 (6.8e-03)\textsuperscript{4}& 4.54e-01 (1.9e-02)\textsuperscript{4}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 1.77e-01 (7.4e-03)\textsuperscript{11}& 2.15e-01 (8.7e-03)\textsuperscript{10}& 4.66e-01 (2.4e-02)\textsuperscript{7}\tabularnewline
&LOESS& 1.72e-01 (5.8e-03)\textsuperscript{9}& 2.13e-01 (7.5e-03)\textsuperscript{7}& 5.13e-01 (2.7e-02)\textsuperscript{8}\tabularnewline
&Isotonic& 1.97e-01 (5.5e-03)\textsuperscript{13}& 2.66e-01 (8.0e-03)\textsuperscript{13}& 9.61e-01 (5.6e-02)\textsuperscript{13}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 1.56e-01 (5.9e-03)\textsuperscript{3}& 1.90e-01 (7.2e-03)\textsuperscript{3}& 4.16e-01 (2.3e-02)\textsuperscript{3}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 1.70e-01 (6.1e-03)\textsuperscript{8}& 2.13e-01 (7.7e-03)\textsuperscript{8}& 5.26e-01 (2.7e-02)\textsuperscript{9}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 1.61e-01 (5.6e-03)\textsuperscript{5}& 1.98e-01 (6.7e-03)\textsuperscript{5}& 4.62e-01 (2.2e-02)\textsuperscript{5}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 1.82e-01 (5.5e-03)\textsuperscript{12}& 2.32e-01 (7.0e-03)\textsuperscript{12}& 5.77e-01 (2.9e-02)\textsuperscript{11}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 1.49e-01 (5.8e-03)\textsuperscript{2}& 1.84e-01 (7.1e-03)\textsuperscript{2}& 4.06e-01 (2.4e-02)\textsuperscript{2}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 1.69e-01 (6.3e-03)\textsuperscript{7}& 2.13e-01 (8.3e-03)\textsuperscript{9}& 5.45e-01 (3.1e-02)\textsuperscript{10}\tabularnewline
\midrule
\multirow{14}{*}{1.5}&Cubic Spline (CS)& 5.47e-01 (3.5e-02)\textsuperscript{14}& 6.88e-01 (4.5e-02)\textsuperscript{14}& 2.00e+00 (1.4e-01)\textsuperscript{14}\tabularnewline
&Monotone CS (MCS)& 2.31e-01 (8.7e-03)\textsuperscript{11}& 2.94e-01 (1.1e-02)\textsuperscript{12}& 9.13e-01 (7.3e-02)\textsuperscript{12}\tabularnewline
&Smoothing Spline (SS)& 2.14e-01 (1.1e-02)\textsuperscript{6}& 2.58e-01 (1.3e-02)\textsuperscript{6}& 5.66e-01 (4.1e-02)\textsuperscript{6}\tabularnewline
&Montone SS (MSS)& \textbf{1.89e-01} (7.8e-03)\textsuperscript{1}& \textbf{2.23e-01} (8.6e-03)\textsuperscript{1}& \textbf{4.59e-01} (2.9e-02)\textsuperscript{1}\tabularnewline
&Quadratic Spline (QS)& 2.05e-01 (8.6e-03)\textsuperscript{2}& 2.47e-01 (9.7e-03)\textsuperscript{5}& 5.48e-01 (2.4e-02)\textsuperscript{4}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 2.27e-01 (1.1e-02)\textsuperscript{8}& 2.77e-01 (1.2e-02)\textsuperscript{8}& 5.87e-01 (3.1e-02)\textsuperscript{8}\tabularnewline
&LOESS& 2.30e-01 (8.8e-03)\textsuperscript{10}& 2.81e-01 (1.1e-02)\textsuperscript{9}& 6.55e-01 (3.0e-02)\textsuperscript{9}\tabularnewline
&Isotonic& 2.62e-01 (8.2e-03)\textsuperscript{13}& 3.52e-01 (1.0e-02)\textsuperscript{13}& 1.34e+00 (6.9e-02)\textsuperscript{13}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 2.06e-01 (8.3e-03)\textsuperscript{4}& 2.46e-01 (9.4e-03)\textsuperscript{3}& 5.25e-01 (2.6e-02)\textsuperscript{2}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 2.29e-01 (8.6e-03)\textsuperscript{9}& 2.82e-01 (1.0e-02)\textsuperscript{10}& 6.98e-01 (3.2e-02)\textsuperscript{10}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016a}: MonoPoly& 2.06e-01 (7.8e-03)\textsuperscript{3}& 2.46e-01 (8.8e-03)\textsuperscript{4}& 5.58e-01 (2.6e-02)\textsuperscript{5}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 2.25e-01 (8.4e-03)\textsuperscript{7}& 2.72e-01 (9.8e-03)\textsuperscript{7}& 5.85e-01 (1.9e-02)\textsuperscript{7}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 2.07e-01 (1.3e-02)\textsuperscript{5}& 2.46e-01 (1.6e-02)\textsuperscript{2}& 5.29e-01 (4.9e-02)\textsuperscript{3}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 2.32e-01 (8.3e-03)\textsuperscript{12}& 2.87e-01 (1.1e-02)\textsuperscript{11}& 7.16e-01 (4.4e-02)\textsuperscript{11}\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/msfe_mspe_logit_growth.tex <==
\begin{tabular}{lllll}
\hline
\toprule
 & \multicolumn{2}{c}{Logistic Curve} & \multicolumn{2}{c}{Growth Curve} \\ 
\cmidrule(lr){2-3}\cmidrule{4-5}
 & \multicolumn{1}{c}{MSFE} & \multicolumn{1}{c}{MSPE} & \multicolumn{1}{c}{MSFE} & \multicolumn{1}{c}{MSPE} \\ 
\midrule
MQB & 2.69e-03 (5.3e-05) & 2.89e-03 (6.1e-05) & 8.32e-01 (2.2e-02) & 7.95e-01 (2.1e-02)\\ 
QB & 2.08e-03 (4.3e-05) & 2.22e-03 (5.3e-05) & 1.18e+00 (2.3e-02) & 1.12e+00 (2.5e-02)\\ 
LOESS & 1.64e-03 (3.1e-05) & 1.70e-03 (3.5e-05) & 8.72e-01 (1.6e-02) & 8.06e-01 (1.8e-02)\\ 
SI & 1.48e-03 (3.0e-05) & 1.61e-03 (3.5e-05) & 8.51e-01 (1.6e-02) & 8.48e-01 (2.0e-02)\\ 
IS & 1.62e-03 (3.2e-05) & 1.74e-03 (3.6e-05) & 8.53e-01 (1.6e-02) & 7.96e-01 (1.8e-02)\\ 
MCB1 & 2.34e-03 (3.4e-05) & 2.56e-03 (3.9e-05) & 4.38e-01 (7.8e-03) & 4.47e-01 (9.2e-03)\\ 
MCB2 & 2.53e-03 (4.2e-05) & 2.81e-03 (5.1e-05) & 5.83e-01 (9.3e-03) & 6.94e-01 (1.5e-02)\\ 
CB1 & 2.05e-03 (3.4e-05) & 2.17e-03 (4.3e-05) & 5.41e-01 (8.8e-03) & 5.73e-01 (1.2e-02)\\ 
CB2 & 5.58e-03 (1.1e-04) & 3.73e+04 (3.2e+04) & 1.32e+00 (2.4e-02) & 3.20e+06 (2.3e+06)\\ 
\bottomrule
\end{tabular}

==> res/mono_fit/msfe_mspe_logit_growth_0.1.tex <==
\begin{tabular}{lllll}
\hline
\toprule
 & \multicolumn{2}{c}{Logistic Curve} & \multicolumn{2}{c}{Growth Curve} \\
\cmidrule(lr){2-3}\cmidrule{4-5}
 & \multicolumn{1}{c}{MSFE} & \multicolumn{1}{c}{MSPE} & \multicolumn{1}{c}{MSFE} & \multicolumn{1}{c}{MSPE} \\
\midrule
MQB & 2.69e-03 (5.3e-05) & 2.85e-03 (5.8e-05) & 9.55e-03 (4.7e-04) & 3.43e-02 (2.9e-03)\\
QB & 2.09e-03 (4.7e-05) & 2.19e-03 (5.4e-05) & 3.81e-02 (2.8e-03) & 7.78e-02 (5.5e-03)\\
LOESS & 1.63e-03 (3.0e-05) & 1.67e-03 (3.3e-05) & 5.41e-01 (1.3e-02) & 4.99e-01 (1.5e-02)\\
SI & \textbf{1.46e-03 (2.9e-05)} & \textbf{1.59e-03 (3.3e-05)} & 5.41e-01 (1.3e-02) & 5.69e-01 (1.9e-02)\\
IS & 1.58e-03 (3.0e-05) & 1.69e-03 (3.4e-05) & 5.41e-01 (1.3e-02) & 4.99e-01 (1.5e-02)\\
MCB1 & 2.24e-03 (3.3e-05) & 2.47e-03 (4.0e-05) & \textbf{5.03e-03 (5.5e-04)} & \textbf{1.46e-02 (1.5e-03)}\\
MCB2 & 2.37e-03 (4.0e-05) & 2.68e-03 (5.3e-05) & 6.27e-03 (6.7e-05) & 9.08e-02 (9.2e-03)\\
CB1 & 2.02e-03 (3.3e-05) & 2.12e-03 (4.5e-05) & 5.05e-03 (3.5e-04) & 1.53e-02 (1.4e-03)\\
CB2 & 5.21e-03 (1.1e-04) & 3.76e+03 (2.1e+03) & 8.62e-03 (9.3e-05) & 1.17e+05 (5.0e+04)\\
\bottomrule
\end{tabular}


==> res/mono_fit/msfe_mspe_logit_growth_1.5.tex <==
\begin{tabular}{lllll}
\hline
\toprule
 & \multicolumn{2}{c}{Logistic Curve} & \multicolumn{2}{c}{Growth Curve} \\
\cmidrule(lr){2-3}\cmidrule{4-5}
 & \multicolumn{1}{c}{MSFE} & \multicolumn{1}{c}{MSPE} & \multicolumn{1}{c}{MSFE} & \multicolumn{1}{c}{MSPE} \\
\midrule
MQB & 2.38e-01 (7.3e-03) & 2.30e-01 (7.0e-03) & 8.83e-01 (2.1e-02) & 8.57e-01 (2.4e-02)\\
QB & 2.47e-01 (6.4e-03) & 2.39e-01 (6.3e-03) & 1.23e+00 (2.4e-02) & 1.19e+00 (2.8e-02)\\
LOESS & 3.53e-01 (7.3e-03) & 3.41e-01 (7.3e-03) & 9.25e-01 (1.6e-02) & 8.72e-01 (2.1e-02)\\
SI & 2.17e-01 (5.6e-03) & 2.05e-01 (5.3e-03) & 9.02e-01 (1.6e-02) & 9.14e-01 (2.4e-02)\\
IS & 2.62e-01 (6.5e-03) & 2.43e-01 (6.0e-03) & 9.01e-01 (1.6e-02) & 8.56e-01 (2.1e-02)\\
MCB1 & \textbf{2.03e-01 (5.7e-03)} & \textbf{1.91e-01 (5.3e-03)} & \textbf{4.63e-01 (8.7e-03)} & \textbf{4.70e-01 (1.0e-02)}\\
MCB2 & 2.72e-01 (7.0e-03) & 2.38e-01 (6.1e-03) & 5.92e-01 (9.5e-03) & 7.03e-01 (1.6e-02)\\
CB1 & 4.02e-01 (9.3e-03) & 3.98e-01 (1.0e-02) & 5.64e-01 (9.4e-03) & 5.91e-01 (1.2e-02)\\
CB2 & 1.02e+00 (2.5e-02) & 2.47e+05 (1.2e+05) & 1.28e+00 (2.4e-02) & 1.69e+05 (8.8e+04)\\
\bottomrule
\end{tabular}


==> res/mono_fit/poly3_2023-09-25T17_54_13-04_00_nrep100.tex <==
\begin{tabular}{ccccc}
\toprule
Noise $\sigma$ & Method&$\frac 1n L_1$&$\frac{1}{\sqrt n}L_2$&$L_\infty$\tabularnewline
\midrule
\multirow{14}{*}{0.1}&Cubic Spline (CS)& 4.25e-02 (2.5e-03)\textsuperscript{14}& 5.31e-02 (3.1e-03)\textsuperscript{14}& 1.43e-01 (9.1e-03)\textsuperscript{13}\tabularnewline
&Monotone CS (MCS)& 2.64e-02 (8.5e-04)\textsuperscript{9}& 3.39e-02 (1.1e-03)\textsuperscript{10}& 9.83e-02 (5.0e-03)\textsuperscript{10}\tabularnewline
&Smoothing Spline (SS)& 2.24e-02 (5.9e-04)\textsuperscript{4}& 2.87e-02 (7.4e-04)\textsuperscript{4}& 8.28e-02 (3.2e-03)\textsuperscript{4}\tabularnewline
&Montone SS (MSS)& 2.09e-02 (5.5e-04)\textsuperscript{3}& 2.72e-02 (6.8e-04)\textsuperscript{3}& 8.17e-02 (3.2e-03)\textsuperscript{3}\tabularnewline
&Quadratic Spline (QS)& 1.93e-02 (4.9e-04)\textsuperscript{2}& 2.41e-02 (6.2e-04)\textsuperscript{2}& 6.19e-02 (2.3e-03)\textsuperscript{2}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 2.49e-02 (6.0e-04)\textsuperscript{5}& 3.13e-02 (8.0e-04)\textsuperscript{5}& 8.52e-02 (4.0e-03)\textsuperscript{5}\tabularnewline
&LOESS& 2.56e-02 (6.1e-04)\textsuperscript{8}& 3.21e-02 (6.7e-04)\textsuperscript{7}& 9.01e-02 (3.0e-03)\textsuperscript{7}\tabularnewline
&Isotonic& 3.40e-02 (4.6e-04)\textsuperscript{12}& 4.52e-02 (6.0e-04)\textsuperscript{12}& 1.47e-01 (3.5e-03)\textsuperscript{14}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 2.53e-02 (6.3e-04)\textsuperscript{7}& 3.18e-02 (6.8e-04)\textsuperscript{6}& 9.01e-02 (3.0e-03)\textsuperscript{8}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 2.73e-02 (6.5e-04)\textsuperscript{10}& 3.39e-02 (6.9e-04)\textsuperscript{9}& 9.08e-02 (3.0e-03)\textsuperscript{9}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016}: MonoPoly& \textbf{1.44e-02} (6.0e-04)\textsuperscript{1}& \textbf{1.77e-02} (6.9e-04)\textsuperscript{1}& \textbf{4.35e-02} (2.0e-03)\textsuperscript{1}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 3.66e-02 (3.3e-03)\textsuperscript{13}& 4.59e-02 (3.9e-03)\textsuperscript{13}& 1.32e-01 (1.0e-02)\textsuperscript{12}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 2.51e-02 (5.2e-04)\textsuperscript{6}& 3.22e-02 (6.5e-04)\textsuperscript{8}& 8.97e-02 (2.8e-03)\textsuperscript{6}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 3.40e-02 (1.0e-03)\textsuperscript{11}& 4.32e-02 (1.3e-03)\textsuperscript{11}& 1.02e-01 (4.0e-03)\textsuperscript{11}\tabularnewline
\midrule
\multirow{14}{*}{1.0}&Cubic Spline (CS)& 3.89e-01 (2.3e-02)\textsuperscript{14}& 4.88e-01 (2.9e-02)\textsuperscript{14}& 1.37e+00 (8.5e-02)\textsuperscript{14}\tabularnewline
&Monotone CS (MCS)& 1.71e-01 (5.5e-03)\textsuperscript{8}& 2.23e-01 (6.7e-03)\textsuperscript{9}& 6.84e-01 (3.7e-02)\textsuperscript{11}\tabularnewline
&Smoothing Spline (SS)& 1.80e-01 (7.1e-03)\textsuperscript{10}& 2.24e-01 (9.0e-03)\textsuperscript{10}& 5.46e-01 (2.8e-02)\textsuperscript{9}\tabularnewline
&Montone SS (MSS)& 1.58e-01 (5.4e-03)\textsuperscript{4}& 2.00e-01 (5.9e-03)\textsuperscript{5}& 4.98e-01 (2.0e-02)\textsuperscript{5}\tabularnewline
&Quadratic Spline (QS)& 1.76e-01 (4.9e-03)\textsuperscript{9}& 2.17e-01 (5.5e-03)\textsuperscript{8}& 5.37e-01 (2.2e-02)\textsuperscript{7}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 1.91e-01 (6.1e-03)\textsuperscript{12}& 2.32e-01 (7.0e-03)\textsuperscript{11}& 5.42e-01 (2.2e-02)\textsuperscript{8}\tabularnewline
&LOESS& 1.68e-01 (5.8e-03)\textsuperscript{7}& 2.04e-01 (7.0e-03)\textsuperscript{6}& 4.76e-01 (2.3e-02)\textsuperscript{4}\tabularnewline
&Isotonic& 1.87e-01 (5.2e-03)\textsuperscript{11}& 2.54e-01 (6.5e-03)\textsuperscript{12}& 8.93e-01 (4.3e-02)\textsuperscript{13}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 1.54e-01 (5.7e-03)\textsuperscript{2}& 1.90e-01 (6.5e-03)\textsuperscript{2}& 4.50e-01 (2.1e-02)\textsuperscript{3}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 1.59e-01 (6.0e-03)\textsuperscript{5}& 1.95e-01 (6.9e-03)\textsuperscript{3}& 4.22e-01 (2.0e-02)\textsuperscript{2}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016}: MonoPoly& \textbf{1.38e-01} (5.6e-03)\textsuperscript{1}& \textbf{1.70e-01} (6.4e-03)\textsuperscript{1}& \textbf{3.98e-01} (1.8e-02)\textsuperscript{1}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 2.48e-01 (5.0e-03)\textsuperscript{13}& 3.06e-01 (4.8e-03)\textsuperscript{13}& 7.44e-01 (2.5e-02)\textsuperscript{12}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 1.57e-01 (5.5e-03)\textsuperscript{3}& 1.98e-01 (6.0e-03)\textsuperscript{4}& 5.01e-01 (2.1e-02)\textsuperscript{6}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 1.67e-01 (6.7e-03)\textsuperscript{6}& 2.14e-01 (8.7e-03)\textsuperscript{7}& 5.67e-01 (3.0e-02)\textsuperscript{10}\tabularnewline
\midrule
\multirow{14}{*}{1.5}&Cubic Spline (CS)& 5.21e-01 (3.4e-02)\textsuperscript{14}& 6.53e-01 (4.1e-02)\textsuperscript{14}& 1.82e+00 (1.3e-01)\textsuperscript{14}\tabularnewline
&Monotone CS (MCS)& 2.38e-01 (8.2e-03)\textsuperscript{6}& 3.12e-01 (1.0e-02)\textsuperscript{10}& 1.00e+00 (6.4e-02)\textsuperscript{12}\tabularnewline
&Smoothing Spline (SS)& 2.40e-01 (1.0e-02)\textsuperscript{8}& 2.96e-01 (1.3e-02)\textsuperscript{6}& 7.10e-01 (3.9e-02)\textsuperscript{5}\tabularnewline
&Montone SS (MSS)& 2.15e-01 (8.0e-03)\textsuperscript{2}& 2.65e-01 (8.9e-03)\textsuperscript{2}& 6.33e-01 (2.7e-02)\textsuperscript{4}\tabularnewline
&Quadratic Spline (QS)& 2.38e-01 (7.9e-03)\textsuperscript{7}& 2.91e-01 (8.9e-03)\textsuperscript{5}& 7.22e-01 (2.6e-02)\textsuperscript{7}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 2.56e-01 (1.0e-02)\textsuperscript{11}& 3.11e-01 (1.2e-02)\textsuperscript{9}& 7.24e-01 (3.1e-02)\textsuperscript{8}\tabularnewline
&LOESS& 2.42e-01 (8.5e-03)\textsuperscript{9}& 2.98e-01 (1.0e-02)\textsuperscript{8}& 7.12e-01 (2.9e-02)\textsuperscript{6}\tabularnewline
&Isotonic& 2.55e-01 (8.4e-03)\textsuperscript{10}& 3.49e-01 (1.1e-02)\textsuperscript{11}& 1.26e+00 (6.6e-02)\textsuperscript{13}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 2.16e-01 (8.2e-03)\textsuperscript{3}& 2.66e-01 (8.8e-03)\textsuperscript{3}& 6.33e-01 (2.3e-02)\textsuperscript{3}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 2.22e-01 (9.4e-03)\textsuperscript{4}& 2.71e-01 (1.1e-02)\textsuperscript{4}& 5.91e-01 (3.1e-02)\textsuperscript{2}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016}: MonoPoly& \textbf{2.02e-01} (8.5e-03)\textsuperscript{1}& \textbf{2.46e-01} (9.4e-03)\textsuperscript{1}& \textbf{5.83e-01} (2.4e-02)\textsuperscript{1}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 2.92e-01 (7.2e-03)\textsuperscript{13}& 3.55e-01 (7.0e-03)\textsuperscript{12}& 8.18e-01 (3.2e-02)\textsuperscript{10}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 2.89e-01 (2.7e-02)\textsuperscript{12}& 3.58e-01 (3.4e-02)\textsuperscript{13}& 8.91e-01 (9.8e-02)\textsuperscript{11}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 2.34e-01 (9.0e-03)\textsuperscript{5}& 2.96e-01 (1.1e-02)\textsuperscript{7}& 7.41e-01 (3.7e-02)\textsuperscript{9}\tabularnewline
\bottomrule
\end{tabular}


==> res/mono_fit/step_2023-09-25T17_54_13-04_00_nrep100.tex <==
\begin{tabular}{ccccc}
\toprule
Noise $\sigma$ & Method&$\frac 1n L_1$&$\frac{1}{\sqrt n}L_2$&$L_\infty$\tabularnewline
\midrule
\multirow{14}{*}{0.1}&Cubic Spline (CS)& 7.65e-02 (6.1e-04)\textsuperscript{5}& 9.67e-02 (7.4e-04)\textsuperscript{3}& 2.78e-01 (4.5e-03)\textsuperscript{2}\tabularnewline
&Monotone CS (MCS)& 4.94e-02 (9.2e-04)\textsuperscript{2}& 8.41e-02 (1.6e-03)\textsuperscript{2}& 3.97e-01 (1.1e-02)\textsuperscript{3}\tabularnewline
&Smoothing Spline (SS)& 7.46e-02 (1.2e-03)\textsuperscript{4}& 1.10e-01 (2.2e-03)\textsuperscript{4}& 4.44e-01 (1.4e-02)\textsuperscript{4}\tabularnewline
&Montone SS (MSS)& 7.29e-02 (1.4e-03)\textsuperscript{3}& 1.26e-01 (2.4e-03)\textsuperscript{5}& 5.33e-01 (1.4e-02)\textsuperscript{5}\tabularnewline
&Quadratic Spline (QS)& 1.95e-01 (3.6e-03)\textsuperscript{9}& 2.68e-01 (5.1e-03)\textsuperscript{9}& 8.69e-01 (2.7e-02)\textsuperscript{8}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 1.59e-01 (3.1e-03)\textsuperscript{7}& 2.56e-01 (3.9e-03)\textsuperscript{8}& 9.85e-01 (3.0e-02)\textsuperscript{9}\tabularnewline
&LOESS& 3.76e-01 (7.7e-03)\textsuperscript{12}& 4.77e-01 (1.0e-02)\textsuperscript{12}& 1.28e+00 (3.5e-02)\textsuperscript{10}\tabularnewline
&Isotonic& \textbf{3.61e-02} (6.6e-04)\textsuperscript{1}& \textbf{4.99e-02} (7.8e-04)\textsuperscript{1}& \textbf{1.84e-01} (5.6e-03)\textsuperscript{1}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 3.75e-01 (7.7e-03)\textsuperscript{11}& 4.76e-01 (1.0e-02)\textsuperscript{11}& 1.28e+00 (3.5e-02)\textsuperscript{11}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 3.77e-01 (7.7e-03)\textsuperscript{13}& 4.78e-01 (1.0e-02)\textsuperscript{13}& 1.28e+00 (3.5e-02)\textsuperscript{12}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016}: MonoPoly& 4.94e-01 (1.5e-02)\textsuperscript{14}& 6.09e-01 (1.8e-02)\textsuperscript{14}& 1.51e+00 (4.4e-02)\textsuperscript{14}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 1.74e-01 (1.1e-02)\textsuperscript{8}& 2.44e-01 (1.2e-02)\textsuperscript{7}& 7.64e-01 (2.9e-02)\textsuperscript{7}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 9.73e-02 (2.0e-03)\textsuperscript{6}& 1.59e-01 (2.9e-03)\textsuperscript{6}& 6.07e-01 (1.5e-02)\textsuperscript{6}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 3.56e-01 (6.1e-03)\textsuperscript{10}& 4.75e-01 (9.4e-03)\textsuperscript{10}& 1.43e+00 (4.6e-02)\textsuperscript{13}\tabularnewline
\midrule
\multirow{14}{*}{1.0}&Cubic Spline (CS)& 5.70e-01 (1.6e-02)\textsuperscript{14}& 7.19e-01 (2.0e-02)\textsuperscript{14}& 2.04e+00 (6.2e-02)\textsuperscript{14}\tabularnewline
&Monotone CS (MCS)& \textbf{3.02e-01} (5.7e-03)\textsuperscript{1}& \textbf{3.92e-01} (6.5e-03)\textsuperscript{1}& 1.17e+00 (3.0e-02)\textsuperscript{3}\tabularnewline
&Smoothing Spline (SS)& 3.31e-01 (5.2e-03)\textsuperscript{5}& 4.16e-01 (6.2e-03)\textsuperscript{5}& 1.18e+00 (2.9e-02)\textsuperscript{4}\tabularnewline
&Montone SS (MSS)& 3.11e-01 (5.6e-03)\textsuperscript{3}& 3.93e-01 (6.5e-03)\textsuperscript{3}& 1.10e+00 (2.3e-02)\textsuperscript{2}\tabularnewline
&Quadratic Spline (QS)& 4.11e-01 (6.9e-03)\textsuperscript{11}& 5.13e-01 (8.6e-03)\textsuperscript{10}& 1.34e+00 (2.9e-02)\textsuperscript{7}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 4.06e-01 (7.2e-03)\textsuperscript{8}& 5.07e-01 (8.6e-03)\textsuperscript{7}& 1.36e+00 (3.1e-02)\textsuperscript{11}\tabularnewline
&LOESS& 4.09e-01 (6.0e-03)\textsuperscript{10}& 5.12e-01 (7.4e-03)\textsuperscript{9}& 1.35e+00 (2.8e-02)\textsuperscript{9}\tabularnewline
&Isotonic& 3.13e-01 (5.7e-03)\textsuperscript{4}& 4.10e-01 (6.7e-03)\textsuperscript{4}& 1.27e+00 (3.1e-02)\textsuperscript{5}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 4.08e-01 (6.0e-03)\textsuperscript{9}& 5.11e-01 (7.3e-03)\textsuperscript{8}& 1.35e+00 (2.8e-02)\textsuperscript{8}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 4.13e-01 (6.0e-03)\textsuperscript{12}& 5.17e-01 (7.4e-03)\textsuperscript{11}& 1.36e+00 (2.8e-02)\textsuperscript{10}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016}: MonoPoly& 4.99e-01 (1.1e-02)\textsuperscript{13}& 6.17e-01 (1.3e-02)\textsuperscript{13}& 1.55e+00 (3.9e-02)\textsuperscript{13}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 3.54e-01 (8.0e-03)\textsuperscript{6}& 4.51e-01 (1.0e-02)\textsuperscript{6}& 1.29e+00 (5.5e-02)\textsuperscript{6}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& 3.10e-01 (5.6e-03)\textsuperscript{2}& 3.92e-01 (6.6e-03)\textsuperscript{2}& \textbf{1.09e+00} (2.4e-02)\textsuperscript{1}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 4.04e-01 (7.9e-03)\textsuperscript{7}& 5.21e-01 (1.0e-02)\textsuperscript{12}& 1.50e+00 (4.5e-02)\textsuperscript{12}\tabularnewline
\midrule
\multirow{14}{*}{1.5}&Cubic Spline (CS)& 7.61e-01 (2.6e-02)\textsuperscript{14}& 9.57e-01 (3.3e-02)\textsuperscript{14}& 2.72e+00 (9.8e-02)\textsuperscript{14}\tabularnewline
&Monotone CS (MCS)& 4.15e-01 (7.4e-03)\textsuperscript{3}& 5.32e-01 (8.4e-03)\textsuperscript{3}& 1.57e+00 (4.6e-02)\textsuperscript{8}\tabularnewline
&Smoothing Spline (SS)& 4.28e-01 (8.4e-03)\textsuperscript{4}& 5.36e-01 (9.9e-03)\textsuperscript{4}& 1.42e+00 (3.2e-02)\textsuperscript{3}\tabularnewline
&Montone SS (MSS)& 4.04e-01 (8.1e-03)\textsuperscript{2}& 5.09e-01 (9.4e-03)\textsuperscript{2}& 1.36e+00 (3.1e-02)\textsuperscript{2}\tabularnewline
&Quadratic Spline (QS)& 4.80e-01 (9.8e-03)\textsuperscript{11}& 5.99e-01 (1.1e-02)\textsuperscript{11}& 1.55e+00 (3.6e-02)\textsuperscript{7}\tabularnewline
&\textcite{heMonotoneBsplineSmoothing1998}: MQS& 5.06e-01 (9.6e-03)\textsuperscript{12}& 6.31e-01 (1.2e-02)\textsuperscript{12}& 1.64e+00 (4.3e-02)\textsuperscript{11}\tabularnewline
&LOESS& 4.52e-01 (8.2e-03)\textsuperscript{8}& 5.69e-01 (1.0e-02)\textsuperscript{8}& 1.49e+00 (3.5e-02)\textsuperscript{6}\tabularnewline
&Isotonic& 4.31e-01 (7.9e-03)\textsuperscript{5}& 5.63e-01 (8.6e-03)\textsuperscript{5}& 1.76e+00 (5.0e-02)\textsuperscript{13}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: SI (LOESS+Isotonic)& 4.50e-01 (8.1e-03)\textsuperscript{7}& 5.65e-01 (9.8e-03)\textsuperscript{6}& 1.49e+00 (3.5e-02)\textsuperscript{5}\tabularnewline
&\textcite{mammenEstimatingSmoothMonotone1991}: IS (Isotonic+LOESS)& 4.57e-01 (7.9e-03)\textsuperscript{9}& 5.72e-01 (9.8e-03)\textsuperscript{9}& 1.48e+00 (3.4e-02)\textsuperscript{4}\tabularnewline
&\textcite{murrayFastFlexibleMethods2016}: MonoPoly& 5.19e-01 (1.4e-02)\textsuperscript{13}& 6.41e-01 (1.6e-02)\textsuperscript{13}& 1.60e+00 (4.0e-02)\textsuperscript{10}\tabularnewline
&\textcite{cannonMonmlpMultilayerPerceptron2017}: MONMLP& 4.61e-01 (1.0e-02)\textsuperscript{10}& 5.88e-01 (1.3e-02)\textsuperscript{10}& 1.70e+00 (5.3e-02)\textsuperscript{12}\tabularnewline
&\textcite{navarro-garciaConstrainedSmoothingOutofrange2023}: cpsplines& \textbf{3.99e-01} (7.6e-03)\textsuperscript{1}& \textbf{5.04e-01} (8.9e-03)\textsuperscript{1}& \textbf{1.35e+00} (3.0e-02)\textsuperscript{1}\tabularnewline
&\textcite{groeneboomConfidenceIntervalsMonotone2023}: SLSE& 4.49e-01 (8.4e-03)\textsuperscript{6}& 5.67e-01 (1.1e-02)\textsuperscript{7}& 1.60e+00 (5.2e-02)\textsuperscript{9}\tabularnewline
\bottomrule
\end{tabular}

